How Two-Layer Neural Networks Learn, One (Giant) Step at a Time

For high-dimensional Gaussian data, we investigate theoretically how the features of a two-layer neural network adapt to the structure of the target function through a few large batch gradient descent steps, leading to an improvement in the approximation capacity from initialization. First, we compare the influence of batch size to that of multiple steps. For a single step, a batch of size $n = \mathcal{O}(d)$ is both necessary and sufficient to align with the target function, although only a single direction can be learned. In contrast, $n = \mathcal{O}(d^2)$ is essential for neurons to specialize in multiple relevant directions of the target with a single gradient step. Even in this case, we show there might exist ``hard'' directions requiring $n = \mathcal{O}(d^\ell)$ samples to be learned, where $\ell$ is known as the leap index of the target. Second, we show that the picture drastically improves over multiple gradient steps: a batch size of $n = \mathcal{O}(d)$ is indeed sufficient to learn multiple target directions satisfying a staircase property, where more and more directions can be learned over time. Finally, we discuss how these directions allow for a drastic improvement in the approximation capacity and generalization error over the initialization, illustrating a separation of scale between the random features/lazy regime and the feature learning regime. Our technical analysis leverages a combination of techniques related to concentration, projection-based conditioning, and Gaussian equivalence, which we believe are of independent interest. By pinning down the conditions necessary for specialization and learning, our results highlight the intertwined role of the structure of the task to learn, the details of the algorithm, and the architecture, shedding new light on how neural networks adapt to the feature and learn complex task from data over time.

==> reviewed_section/investigation.tex <==





% \begin{figure}[t]
%     \centering
%     \includegraphics[width = 1\textwidth]{figs/multiple_steps.pdf}
% %    \vspace{-10em}
%     \caption{{\bf The gradient after multiple steps:}   \lp{Will be put after multiple GD statement. If the proof problem for multiple GD steps cannot be settled, this will be numerics in support of a conjecture for $T<c \log{d}$.} Illustration of the lack of specialization after finite number of GD steps in the proportional regime $n = \mathcal{O}(d)$. We study the cosine similarity with respect to the teacher vectors $(\vec{\theta}_1,\vec{\theta}_2)$ for the gradient of $2$ different neurons (identified respectively by a square and triangle). We fix the relevant dimension $(n,d,p) = (2^{13},2^{13},2^{6})$,  and we perform $15$ GD steps with a fixed learning rate $\eta = \sqrt{p}$. We plot the predicted orientation for the neurons in the teacher subspace as a continuous red line, while the bisectrix of the first quadrant is in a dashed black line. We draw the circle of unitary radius in black, if the gradient was perfectly correlated with the teachers, the neurons would lie on the circumference. On the other hand, the green circle is of radius $\sfrac{2}{\sqrt{d}}$, if the gradient was completely uncorrelated with the teacher, the neurons would lie approximately inside the latter circle. The purple boxes are the end-points for perfectly specialized neurons. We consider different teacher-student settings by fixing the student non-linearity to be $\sigma(z) = \rm{relu}(z)$ and varying the teacher ones for the different sections. Let for simplicity $s(z) = 4z+z^2$, we have: \textbf{Left:} $\sigma_1^*(z) = z, \sigma^*_2(z) = s(z)$. \textbf{Center:} $\sigma_1^*(z) = \sigma^*_2(z) = s(z)$. \textbf{Right:} $\sigma_1^*(z) = s(z), \sigma^*_2(z) = z $.}
%     \label{fig:no_spec}
% \end{figure}


==> sections/intro.tex <==
%{\bf TODO  : 
%\begin{itemize}
%\item Mention the link with saddle to saddle, "one (near) saddle at a time".
%\item More ref to information exponent, and leap exponentnt, uniftyin a bit
%\item Kernel/Random feature conjecture needed clarification, add the example we had in the talk
%\item Mention the tradeoff in computation al complexity : with respect to SGD we loose a factor d BUT we win a time order one
%\end{itemize}
%}

A central property behind the success of neural networks is their capacity to adapt to the features in the training data. Indeed, many of the classical machine learning methods, e.g. linear or logistic regression, are specifically designed to a restricted class of functions (e.g. generalized linear functions). Others, such as kernel methods, can adapt to larger function classes (e.g. square-integrable functions), but sometimes at prohibitively many samples. Despite the limitations, these methods enjoy well-understood theoretical guarantees: they are convex (hence easy to train) and given a target function, it is well-understood how many samples are needed to achieve a target accuracy. The situation is dramatically different for neural networks: despite being universal approximators, little is known on how to optimally train them or how many hidden units and/or samples are required to learn a given class of functions. Nevertheless, they have proven to be flexible, efficient and easy to optimize in practice, properties which are often attributed to their capacity to adapt to features in the data. Curiously, most of our current theoretical understanding of neural networks stems from the investigation of their lazy regime where features are {\it not} learned during training. In this work, we take some (giant) steps forward from the lazy regime.

% A number of theoretical efforts have been directed toward understanding the dynamics of training neural networks with gradient descent, aiming to uncover the underlying principles that govern their learning capabilities. By iteratively adjusting the network's weights based on the gradients of a chosen objective function, gradient descent seeks to minimize the discrepancy between predicted and true outputs. In this process, the network adapts to the data, learning which features in the input data are most important for explaining the labels. This adaptivity is in contrast to other machine learning pipelines such as random feature or kernel methods,  and is behind the success of neural networks in efficiently solving problems from image classification to text generation.

%In this paper, we delve into the training dynamics of shallow neural networks, focusing on the conditions that facilitate effective feature learning beyond the kernel or random features regime. We aim to answer the following fundamental question: can we precisely capture the presence of feature learning in the {\it early phase} of gradient descent training? We shall thus investigate how the {\it very first few gradient steps} on the first-layer parameters impact the representation abilities. Given we only perform  a few steps, it will have to be giant ones, and we will use large, aggressive, learning rates.

% ADD SOMETHING ALONS THE LINE OF THE 


Our central goal is to paint a complete picture of how two-layer neural networks adapt to the features of training data $(\vec{z}^\nu, y^\nu)_{\nu=1}^{n}\in\mathbb{R}^{d+1}$ in the {\it early phase} of training after the first few steps of gradient descent. We recall the reader that for data is supported in a high-dimensional space, the curse of dimensionality prevents efficient learning even under standard regularity assumptions on the target function such as Lipschitzness \citep{devroye2013probabilistic}.
Hence, understanding the efficient learning performance of neural networks observed in practice requires additional assumptions on the data distribution. In this work, we focus on a popular synthetic data model consisting of: a) independently drawn standard Gaussian covariates $\vec{z}^{\nu}\sim\cN(0, I_d)$; b) a target function $y^{\nu}=f^\star(\vec{z}^{\nu})$ depending only on a finite number of relevant directions, also known as a \emph{multi-index model}. In other words, there exists a finite number of orthogonal \emph{teacher vectors} $\vec{w}_1^\star, \dots, \vec{w}_r^\star$ such that
    \begin{equation}
        y = f^\star(\vec{z}) \coloneqq g^\star(\langle\vec{w_1}^\star,\vec{z}\rangle,\dots, \langle\vec{w_r}^\star,\vec{z}\rangle).
    \end{equation}
 Note that in this model the features are isotropic, with all the structure in the data being in the target. In contrast to other popular models for structured data , such as low-dimensional support of the inputs or smoothness of the target function, kernel methods do not adapt to target functions depending on low-dimensional projections \cite{bach2017breaking}. This makes it an ideal playground for quantifying the adaptativity of neural networks in the feature-learning regime. Given this class of structured targets, we consider supervised learning with the simplest universal approximator neural network: a fully-connected two-layer network with first and second layer weights $W \in \dR^{p\times d}$ and $\vec{a}\in \dR^p$ and activation function  $\sigma:\mathbb{R}\to\mathbb{R}$:
\begin{align}\label{eq:def_2lnn}
    \hat f(\vec{z}; W, \vec{a}) = \frac1{\sqrt{p}}\sum_{i = 1}^{p} a_i \sigma(\langle \vec{w}_i, \vec{z} \rangle).
\end{align}
The primary focus of this work is to elucidate how a two-layer neural network adapts to a low-dimensional target structure during its training. We aim to understand the interplay among the structure of the task (specifically, the complexity of the hidden true function), the details of the algorithm (here the batch size), and the architecture (the number of hidden neurons) in the process of learning from data \citep{zdeborova2020understanding}. In particular, we will be interested in quantifying how much data is required for the relevant directions of the target to be learned, and how this feature learning translates into the approximation capacity of the network with respect to kernel methods.

%\fk{Few words on the fact that we do single pass, and batch size $n=d^l$, Maybe motivate the setting by federated learning and modern practice, maybe cite work such as 
%\cite{goyal2017accurate,li2020review} and others.}.... 

%Our results highlight the fundamental role of batch-size in feature learning, and its interplay with the number of epochs and the complexity of the underlying target function. We uncover the presence of a hierarchy in the way two-layer neural networks learn different relevant directions of the target, in terms of their relative weights with respect to the Hermite decomposition of the target, as illustrated in Fig.~\ref{fig:stairway} (for a single steps) and Fig.~\ref{fig:stairway2} (for multiple steps). More precisely, our results can be summarized as follows.

%\bl{Expand this in terms of "learning representations" vs. "learning features".}

%\newpage
\section{Summary of main results}
\begin{wrapfigure}{r}{0.45\textwidth}
  \vspace{-1.cm}
\includegraphics[width=0.44\textwidth]{figs/Fig1_new.jpeg}
  \caption{\textbf{Learning with a single gradient step.} 
  Illustration of the relationship between batch size and target function complexity for learning multi-index functions with a single giant step in the  $n=\Theta(d^k)$ regime (Thms.~\ref{thm:one_step_lower_bound} \& \ref{thm:one_step_learning}). 
  % What can be learned after a single giant gradient steps with $n=\Theta(d^r)$ samples (see text and theorems \ref{thm:one_step_lower_bound} \& \ref{thm:one_step_learning}).
  }
  \label{fig:fig_1}
  \vspace{-0.5cm}
\end{wrapfigure}
%In section \ref{res:generalisation} we show that 
To outperform the network at initialization (which can be regarded as a kernel method) the network must adapt to the data distribution. Mathematically, this translates to developing correlation in the first layer weights with the target directions $\vec{w}^{\star}_{1},\ldots,\vec{w}^{\star}_{r}$. Our first set of results thus precisely focus on {\bf feature learning}, i.e. how the subspace
\[ V^\star \coloneqq \vect(\vec{w}_1, \dots, \vec{w}_r)\]
is learned during training.


\subsection{A single Gradient step} 
First, we discuss the case of {\bf a single gradient step} of {\bf full-batch gradient descent}, which turns out to be already non-trivial \citep{ba2022high,damian2022neural} 
 and consider the update: \begin{equation}\label{eq:first_layer_gd1}
     \vec{w}_i^{1} = \vec{w}_i^0 -  \frac{\eta}{2n} \sum_{\nu = 1}^n \nabla_{\vec{w}_{i}} \left(y^\nu-\hat f(\vec{z}^\nu; W^0, \vec{a}^{0})\right)^{2}\,.
    \end{equation} 
Theorems \ref{thm:one_step_lower_bound} and \ref{thm:one_step_learning} identify a fundamental interplay between batch size and the complexity of the underlying target function. They are summarized in Fig.~\ref{fig:fig_1} (and a particular numerical example is shown in Fig.~\ref{fig:example}). More precisely:

\begin{itemize}
[noitemsep,leftmargin=1em,wide=0pt]
\item We show that developing meaningful correlation with the target function requires a large batch size $n = \cO(d)$ and learning rate $\eta=\Theta(p)$ when $p,d,n$ are large. However, feature learning remains limited in this regime since we prove only a {\it single} direction can be learned. Thus, if the target depends on several relevant directions, only a "single neuron" approximation can be learned.
%\end{itemize}
%\vspace{-0.4cm}

%\begin{itemize}[noitemsep,leftmargin=1em,wide=0pt]
\item Surpassing the single direction approximation with a single step {\it requires} a larger batch size with {\it at least} $n = \cO(d^2)$ samples. This allows for the network weights to {\it specialize} to multiple target directions. 
%Applying a pre-processing that removes the main learned direction, we show that with a batch size of $n = \cO(d^2)$ the gradient spans the space of many directions, allowing for the network weights to {\it specialize} to multiple target directions. 
\item Nonetheless, we show that there might be {\it hard} directions in the target which cannot be learned with $n = \cO(d^2)$. Learning these directions necessitates a batch size of at least $n = \cO(d^\ell)$, as well as suppressing the directions learned at  $n = \cO(d^{\ell-1})$, where $\ell$ is the \emph{leap index} of the target (precisely defined in Def. \ref{def:leap}) that thoroughly speaking corresponds to the lowest non-zero degree of the Hermite polynomials in the expansion of the target in this directions.  
%\item This result allows to contrast the performances of SGD with full-batch SGD. Indeed, \cite{BenArous2021} showed that learning a single-index ($k=1$) target function with one-pass SGD requires $n=\tau=\cO(n^{\ell-1})$ samples and iterations, where the \emph{information exponent} $\ell$ of the target is given by the degree of the first non-zero polynomial in its Hermite decomposition. In contrast, here we see that a full batch gradient  (which can be efficiently paralelized by distributing over many computers) can achieve the same results {\it in a single iteration}, at the price of using $n=\cO(d^{\ell})$ samples instead.
\end{itemize}
This description paints a clear picture on how the role of the batch size, of the learning rate, and the structure of the hidden function are intertwined. The complexity of learning a low-dimensional target function  is a topic that recently saw a surge of interest, and it is thus interesting to contrast these rates with recent results in the litterature.

For a single-index function with leap index $\ell$, one-pass SGD has a sample complexity of $\cO(d^{\ell - 1})$ \citep{BenArous2021}, and it has been recently shown that a smoothed version of SGD achieves a sample complexity of $\cO(d^{\ell/2})$ \citep{damian_2023_smoothing}. This matches a lower bound from the correlation statistical query family, which encompasses all SGD-like methods. In our single step setting,  the sample complexity for large batch learning is $\cO(d^\ell)$, which is worse than both the aforementioned methods. However, the time complexity of each algorithm paints a different picture. Both SGD algorithms are sequential, and require $\cO(d)$ operations per step, which leads to a total time complexity of $\cO(d^{\ell/2 + 1})$ at least. On the other hand, the computation of the update in Eq. \ref{alg:gd_training} is simply an average of independent terms, which is easy to parallelize. Including the time to compute the average of each term e.g. using a \emph{Gossip algorithm} \citep{boyd_2006_randomized}, this sums up to a time complexity of $\cO(d + \log(n))$. Such an algorithm is also amenable to decentralized learning schemes, where each agent only has access to a fraction of the overall data. 

\subsection{Learning over many GD iterations}
The situation drastically improves when taking for {\bf multiple gradient steps}. In this case, focusing on the linear batch size $n={\cal O}(d)$ regime, and using a fresh batch of data at each GD iteration: 
\begin{equation}\label{eq:first_layer_gd}
        \vec{w}_i^{t+1} = \vec{w}_i^t -  \frac{\eta}{2n} \sum_{\nu = 1}^{n} \nabla_{\vec{w}_i} \left(y^\nu-\hat f(\vec{z}^\nu; W^t, \vec{a}^{0})\right)^{2}\,,
    \end{equation}
Note that splitting the training of the first and second layers and using a fresh batch of data at each iteration is a common approximation in this literature \citep{damian2022neural, ba2022high, Bietti2022}. In contrast to the recent works considering the population limit, we stress that here we take the batch size $n$ to scale with the dimension $d$. In the realm of distributed and federated learning, scenarios with large batches, a single pass, and few iterations are often the norm \citep{goyal2017accurate,li2020review} (for instance this is the case when training large language models), further underlining the relevance of this scenario. In this case, Theorem \ref{thm:staircase} shows that more complex subspaces of the target directions {\it may} be progressively learned at each iteration, as we illustrate in Fig. \ref{fig:fig_2}. More precisely:

\begin{itemize}[noitemsep,leftmargin=1em,wide=0pt]
\item Each additional gradient step allows for learning new perpendicular directions {\bf upon the important condition that they are linearly connected to the previously learned directions} (see Sec~.\ref{sec:few-giant-steps} for precise definitions of this staircase property). Therefore, in contrast with a single step, taking multiple steps allows to learn a multiple-index target with only $n={\cal O}(d)$ samples.
\item Nonetheless, directions that are not coupled through the staircase property and with zero first Hermite coefficient cannot be learned in any finite number of steps. In fact, as discussed previously, they require a batch size of at least $n={\cal O}(d^2)$. In other words, while multiple steps help specialization, it cannot help learning ``hard'' target directions.
\end{itemize}

\begin{figure}[t]
\centering
\includegraphics[width=0.95\textwidth]{figs/Fig2_new.jpeg}
\caption{\textbf{Learning with multiple gradient steps.} An illustration of how neural networks trained using $n=\cO(d)$ batches learn relevant directions after multiple GD training steps, allowing to learn more complex functions over time (see Thm. \ref{thm:staircase}). Here we represent the space $V^\star$ of the relevant direction of the target function, and the (normalized) projection of learned direction $W^t$ by the networks for different task $f^\star(\cdot)$ - the function $g(\cdot)$ and $h(\cdot)$ are assumed to have zero first two Hermite coefficients. During the early stage of training, neural networks first learn first a single direction associated to the linear part of the target, and then can learn over time other directions that are linear conditioned on the previous learned ones. Let $\{\vec e_i\}_{i \in [d]}$ be the standard basis of $\mathbb{R}^d$, the four examples show cases where: \textbf{Top left:} No directions is learned at all. \textbf{Top right:} The network can only learn a single direction $\vec e_1$ (single index regime). \textbf{Bottom left:} The network learns a new direction each time, $\vec e_1$, then $\vec e_2$ and finally $\vec e_3$. \textbf{Bottom right:} The network learns $\vec e_1$ at the first step and both $\vec e_2$ and $\vec e_3$ at the second steps.}
\label{fig:fig_2}
\end{figure}
These results warrant the following comments in context of the state of art. First, \cite{abbe2023sgd} (following \cite{abbe2021staircase,abbe2022merged} who introduced staircase functions) generalized the approach of 
\citep{BenArous2021} and showed that (one-sample at a time) SGD can indeed learn staircase functions with $O(d)$ iterations and $O(d)$ samples. Using, as we do here, large batches $n_d=O(d)$ gives the same  $O(d)$ dependence in terms of sample complexity, but allows us to learn them with $O(1)$ iterations instead. This is a nice illustration of the speed-up provided by batch-GD over SGD, as well as how large batch SGD benefits from multiple iterations over a single one (see table \ref{table} for a summary).

Secondly, we note that similar to the \emph{saddle-to-saddle} dynamics under gradient flow \citep{jacot2021saddle,abbe2023sgd,boursier2022gradient}, the dynamics described through Thm.\ref{thm:staircase} involves sequential learning of directions.  We note, however, that in the one-sample SGD regime \citep{BenArous2021,abbe2023sgd} the gradient has vanishing correlation with new directions, thus requiring a polynomial number of updates to escape saddles. In contrast, the large-batch gradient updates contain a finite fraction of components along the new directions, allowing their learning through a single step. Moreover, we show that each update leads to a $\cO(1)$ change in the components along direction in $V^\star$, obviating the need for coordinate-wise projections in \cite{abbe2023sgd}.

The set of results described above provide a mathematical theory on how neural networks learn representations of the data over training. They corroborate, among others, the findings of \cite{kalimeris2019sgd}, who observed that neural networks first fits the best linear classifier and subsequently learns functions of increasing complexity.

\begin{figure}[t]
    \centering    
\includegraphics[width = 0.48\textwidth]{figs/check_positive_cget_vary_alpha_ctrl=easy.pdf}
\includegraphics[width = 0.48\textwidth]{figs/check_positive_cget_vary_alpha_ctrl=difficult.pdf}
    \caption{{\bf Feature learning and generalization:} We illustrate how one step of gradient descent may (or may not) improve generalization over random features. The plot shows the generalization error as a function of the number of hidden neurons $p$ normalized by the number of samples used for the first layer training $n=\{4d,8d,16d\}$ with fixed dimension $d=2^8
$. 
    \textbf{Left}: $f^\star(\vec z)=z_1+z_1 z_2$. While random features can only fit a linear model in the proportional regime considered, one step of gradient descent over $W$ allows to fit the $z_1 z_2$ part, resulting in a much lower generalization error with respect to random features, despite only the direction $z_1$ being learned in $W$.
    \textbf{Right}: $f^\star(\vec z) = z_1+ z_2z_3$. In this case, since the nonlinear part does not depend on $z_1$, one step of gradient descent on the $W$ does not allow to improve generalization over random features (see Theorem \ref{thm:cget} and Corollary \ref{corr:lower_bound}). We refer to App.~\ref{sec:appendix:numerics} for details on the numerics.}
    \label{fig:features}
\end{figure}

\subsection{From features to generalization}
Our last set of results connects feature learning with the approximation capacity of the network and illustrates that feature learning improves the learning of the target function $f^{\star}$ over random initialization.

\begin{itemize}[noitemsep,leftmargin=1em,wide=0pt]
\item We show that a two-layer network with a finite second layer can {\it only} learn the part of the target function in the learned subspace (see Proposition \ref{prop:fixed_width_lower_bound}). In fact, we conjecture that with $p$ large enough (but still finite), it should be possible to approximate this part of $f^{\star}$ up to arbitrary precision (Conj. \ref{conj:approxim_conj}).
\item As (possibly) universal kernels, large width two-layer networks at initialization enjoy of better approximation capacity. Indeed, \cite{mei_generalization_2022} proved that at initialization $W^{t=0}$, with $n=\Theta(d^k)$ only a degree $k$ approximation of the target function can be learned. Our results characterize how feature learning allows us to improve over this sample complexity. In particular, we show that in the directions learned by the first layer, the target function $f^{\star}$ can be learned with less samples, while the component of $f^{\star}$ orthogonal to the learned features still requires $n=\cO(d^{k})$. While a complete mathematical control of the generalization error rates remains a difficult problem (see Conjecture \ref{conj:kernel+feature}), our results provide a clear separation on scales between two-layer networks and NTK-like methods, improving over the state-of-the art in the literature. 

\item In particular, in Corollary \ref{corr:lower_bound} we prove that with a single gradient step and $n,p=\mathcal{O}(d)$, one can {\it only} learn features in this one-dimensional subspace, doing no better than kernels in the orthogonal direction. This is illustrated in Fig.\ref{fig:features} where we give an example where one step of gradient drastically improves generalization, and one where it does not. To prove these results, we provide a stronger {\it conditional} version of the Gaussian equivalence theorem \citep{mei_generalization_2022,goldt_gaussian_2021,hu2022universality}, which is the backbone of Theorem \ref{thm:cget}, and we believe is of independent interest. 
\end{itemize}

The code to reproduce our figures is available on   \href{https://github.com/lucpoisson/GiantStep}{GitHub}, and we refer to App.~\ref{sec:appendix:numerics} for details on the numerical implementations. Proofs are detailed in App.~\ref{sec:appendix:gd_proofs} and App.~\ref{sec:appendix:cget_proofs}.

\paragraph{Other related works ---}
The analysis of high-dimensional asymptotics of kernel regression has provided valuable insights into the advantages and limitations of kernel methods \citep{Dietrich1999, Opper2001, Ghorbani2019, Ghorbani2020, Donhauser2021, Mei2023, Spigler2020, bordelon20a, Canatar2021, simon2022eigenlearning, Cui2021, Cui2022, xiao2022precise}. In particular, a similar stairway picture as in Fig.~\ref{fig:fig_2} emerged from these works \cite{xiao2022precise}. The key difference, however, is that at each regime $n={\cal O}(d^{k})$, kernels can only learn the $k$-th Hermite polynomial of the target. This should be contrasted with our feature learning regime where, once a direction is learned, all its Hermite coefficients are learned. Feature learning corrections to kernel methods have been investigated in \cite{pmlr-v75-dudeja18a, Naveh2021, Seroussi2023, atanasov2022neural, Bietti2022, bordelon2023dynamics, petrini2022learning}. On a complementary line of work, exact asymptotic results for the the random features models have been derived in the literature \citep{mei_generalization_2022, gerace_generalisation_2020, Dhifallah2020, loureiro_learning_2021, loureiro22a, schroder2023deterministic, bosch2023precise}. A large part of these results are enabled by the Gaussian equivalence property \citep{goldt_gaussian_2021, hu2022universality, Montanari2022, dandi2023universality}.

Closer to us are \citep{ba2022high, damian2022neural}. \cite{ba2022high} showed that a sufficiently large single gradient step allows to beat kernel methods. \cite{ba2022high}
showed that a single gradient step yields an approximately rank-one change on the weights which is enough to beat kernel methods, but did not characterize the impact on the generalization error. In our work, we prove that with a single gradient step and $n,p=\mathcal{O}(d)$, one can only learn features in this one-dimensional subspace, doing no better than kernels in the orthogonal direction. Additionally, their results are limited to single-index target and to a single gradient step. In contrast, \cite{damian2022neural} showed that with $n = \omega(d^2)$ samples, two-layer neural networks can specialize to more than one direction of a multi-index target function with zero first Hermite coefficient ($\ell$=2), and were again limited to a single step.
Our work extends their sufficient conditions on the sample complexity to general $\ell\geq 1$. We also show they are also necessary, i.e. $\forall \epsilon >0$, with less data $n = \Theta(d^{\ell-\epsilon})$ one cannot do better than random features. Thus, our results prove a clear separation between the class of functions learned within the $\Theta(d)$ batch-size setting of \cite{ba2022high} and the $\Theta(d^2)$ batch-size setting of \cite{damian_2023_smoothing} and establish a general hierarchy of functions requiring increasing batch-size to be learned with a gradient step. Additionally, we characterize which class of multi-index targets can be instead learned with $n=\cO(d)$ with {\it multiple} steps.

%Here, we build on their results and consider multi-index targets and multiple steps. \cite{damian2022neural} proved that a batch size of $n=\omega(d^2)$ is \emph{sufficient} for learning multiple directions of a multi-index target. However, they did not establish whether this batch size is \emph{necessary}, and were again limited to a single step. Our results reveal that a batch size of $n=\cO(d^2)$ is indeed necessary for learning multiple directions in a single step, and we characterize which class of multi-index targets can be instead learned with $n=\cO(d)$ with multiple steps.

In a related but different vein, \cite{abbe2022merged}, building upon the earlier work of \cite{abbe2021staircase} show how a ``staircase" property of target functions characterizes the sample complexity for infinite width two-layer networks trained by SGD, a.k.a. the mean-field regime \cite{mei2018mean,chizat2018global,rotskoff2018trainability,sirignano2020mean}). Their focus, however, was on the peculiar case of {\it sparse boolean functions} depending solely on linear coefficients, without considering direction-specific specialization. 
% Can maybe add: \cite{abbe2022merged} also considered the setting of mean-field dynamics under a finite number of steps with large batch-size. Their analysis however, results in requiring $n/d$ to grow unbounded for reaching arbitrary accuracy $\epsilon$
More recently, \cite{abbe2023sgd} provided partial results for the case of isotropic Gaussian data, always in the regime of one-pass SGD, involving basis-dependent projections. 
%Maybe we can say that their algorithm requires knowledge of the subspace V^\star
Here we consider the more generic case of multi-index target functions with Gaussian data with large-batch SGD, without the use of a knowledge of the basis, and show that a ``directional staircase" behavior arises when iterating a few giant gradient steps, while a related, but definitely different, picture arises with single steps depending on the batch size. We also provide a sharp characterization of when this phenomenon appears for multi-index targets and networks trained under large batch SGD, and provide a bound on the resulting generalization error.

Similar to the ``summary statistics" approach in \cite{saad.solla_1995_line,BenArous2021,ben2022high}, our analysis is based upon the concentration of the overlaps of the neurons with the target subspace and their norms, instead of the concentration of the full gradient vector considered in recent works such as \cite{abbe2022merged,damian2022neural}, removing any requirements on the constants in the sample complexity
for alignment along the target subspace. 
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.95\textwidth]{figs/Stairway-1.jpg}
%\caption{{\bf Learning with a single gradient step:} Illustration of the relationship between batch size and learning multi-index functions with a single giant steps with learning rate $\cO(p\sqrt{n/d})$, showcasing the stairway to generalization phenomenon: (a) a batch size of $n = \cO(d)$ results in learning only a single direction, approximating the target function with a single index function, (b) a larger batch size of $n = \cO(d^2)$ facilitates specialization, allowing for learning multiple directions and coupling to all their Hermite coefficients, though directions with a null second Hermite coefficient remain unseen, (c) employing $n = \cO(d^3)$ enables learning hard directions with the first nonzero coefficient of 3-degree (light blue neurons) and more generally, directions with $\ell$-Hermite coefficient zero require a batch size of $n = \cO(d^\ell)$. (hard blue neurons)}
%\label{fig:stairway}
%\vspace{-1em}
%\end{figure}



%\begin{figure}[t]
%\centering
%\includegraphics[width=0.95\textwidth]{figs/Stairway-2.jpg}
%\caption{{\bf Learning with a few gradient steps:} Illustration of the staircase phenomenon when using few giants steps  with learning rate $\cO(p\sqrt{n/d})$ in the linear regime $n\approx d$. Upon iteration, one can learn more directions, one at a time, but {\it only}  in the subspace of directions “linearly connected” in the Hermite basis to the learned directions of the previous time-step (see text). In contrast to Fig.~\ref{fig:stairway}, this allows to generalize with multiple directions with $\cO(n)$ batches and does not require cancellation of previous directions, but this specialization is restricted to staircase functions (and "hard" neurons with zero first Hermite coefficients still require $\cO(d^2)$ samples).}
%\label{fig:stairway2}
%\vspace{-1em}
%\end{figure}


% \ls{Move the following paragraphs to the beginning of the "Main results" section ? and remove the summary ?}
% \paragraph{Hermite expansion ---} We recall a few definition and facts that will be useful for stating our results. Given the Gaussian measure $\gamma_m$ on $\dR^m$, we can build a scalar product on $\ell^2(\dR^m, \gamma_m)$ as
% \begin{equation}
%     \langle f, g \rangle_\gamma = \int_{\dR^m} f g \ \mathrm{d} \gamma_m = \dE_{\vec{z}\sim \cN(\vec{0}, I_m)}[f(\vec{z})g(\vec{z})].
% \end{equation}
% It turns out that there is a specific orthonormal basis of interest for this scalar product, that we present in tensor form:
% \begin{definition}\label{def:hermite}
%     Let $f: \dR^m \to \dR$ be a function that is square integrable w.r.t the Gaussian measure. There exists a family of tensors $(C_k(f))_{k\in\dN}$ such that $C_k(f)$ is of order $k$ and for all $\vec{x} \in \dR^m$,
%     \begin{equation}
%         f(\vec{x}) = \sum_{k \in \dN} \langle C_k(f), \cH_k(\vec{x}) \rangle
%     \end{equation}
%     where $\cH_k(\vec{x})$ is the $k$-th order Hermite tensor \citep{grad_1949_note}. Up to symmetry, the tensors $\cH_k(\vec{x})$ are an orthonormal basis of $\ell^2(\dR^m, \gamma)$, in the sense that for any $\vec{i}, \vec{j} \in \dR^k$,
%     \begin{equation}\label{eq:hilbert_orthonormal}
%         \langle \cH_{k, \vec{i}}(\vec{x}), \cH_{k, \vec{j}}(\vec{x}) \rangle_{\gamma} = \frac{1}{|\mathfrak{o}(\vec{i})|} \ind_{\vec{i} \text{ is a permutation of } \vec{j}}
%     \end{equation}
%     where $|\mathfrak{o}(\vec{i})|$ is the number of distinct permutations of $\vec{i}$.
% \end{definition}
% It can be checked from the definition in \cite{grad_1949_note} that the $\cH_k$, and hence the $C_k(f)$, are basis-invariant, and hence represent an actual $k$-linear form on $\dR^m$. Further, the property \eqref{eq:hilbert_orthonormal} yields an immediate expression for the scalar product in $\ell^2(\dR^m, \gamma_m)$:
% \begin{equation}
%     \langle f, g \rangle_\gamma = \sum_{k \in \dN} \langle C_k(f), C_k(g) \rangle.
% \end{equation}

% \paragraph{Higher-order singular value decomposition}

% The higher-order singular value decomposition (HOSVD) of a tensor is defined as follows:
% \begin{definition}[Higher-order SVD]
%     Let $C \in \dR^{m^k}$ be a symmetric tensor of order $k$. A higher-order SVD of $C$ is an orthonormal set $(\vec{u}_1, \dots, \vec{u}_r)$ of $r \leq k$ vectors, as well as a tensor $S \in \dR^{r^k}$ such that
%     \begin{equation}
%         C = \sum_{j_1, \dots, j_k = 1}^r S_{j_1, \dots, j_k} \vec{u}_{j_1} \otimes \dots \otimes \vec{u}_{j_k}
%     \end{equation} 
% \end{definition}
% The singular values tensor $S$, as well as the rank $r$, are unique, but just as the regular SVD, the vectors $(\vec{u}_1, \dots, \vec{u}_r)$ are only unique up to rotations.


% \paragraph{Summary of main results ---}
% Our first set of results discuss the case of {\bf a single gradient step}, which are illustrated in Fig.~\ref{fig:stairway} (A particular numerical example is shown in Fig.~\ref{fig:example}). In this case:
% \begin{itemize}[noitemsep,leftmargin=1em,wide=0pt]
% \item For a large batch size $n = \cO(d)$ and learning rate $\eta={\cal O}(p\sqrt{n/d})$, meaningful feature learning can be obtained that surpasses random features. However, this is limited in that only a {\it single} direction can be learned. Thus, if $r > 1$, only a single-neuron approximation of the target function will be obtained, specifically for the directions with non-zero Hermite coefficients.
% \item Surpassing the single direction approximation {\it requires} utilizing a larger batch size of dimension $n = \cO(d^2)$. Suppressing the main learned direction, we show that with a batch size of $n = \cO(d^2)$ the gradient spans the space of many directions. This allows for the {\it specialization} of the network weights, that is, learning multiple directions. In these directions, the learning process couples {\it all} the non-zero Hermite coefficients of the target function.
% \item Nonetheless, the ``hard'' directions (those for which the first $\ell$ Hermite coefficients are zero), will continue to be disregarded. Learning these directions necessitates a batch size of $n = \cO(d^\ell)$, as well as suppressing the directions learned at  $n = \cO(d^{\ell-1})$.
% \end{itemize}

% The situation drastically changes when allowing for {\bf multiple gradient steps}. In this case, focusing on the linear batch size $n={\cal O}(d)$ regime, the phenomenology, as illustrated in Fig.~\ref{fig:stairway2}, is as follows:
% \begin{itemize}[noitemsep,leftmargin=1em,wide=0pt]
% \item While with a single step we can only learn a single direction in the teacher space, each additional gradient step allows for learning a new perpendicular direction, one at a time, upon the important condition that these directions are coupled through a staircase property (see sec.\ref{sec:few-giant-steps} for details and definitions). Therefore, taking multiple steps allows to learn a multiple-index target with only $n={\cal O}(d)$ data, provided the staircase condition is met.
% \item However, directions that are not coupled through the staircase and with zero first Hermite coefficient cannot be learned in any finite number of steps. In fact, as discussed previously they require a batch size of $n={\cal O}(d^2)$. In other words, while multiple steps help specialization, they do not allow for the identification of ``hard'' target directions.
% \end{itemize}
% %
% We note that aside from the difference in the specialization capacity, taking a single or multiple steps have an important difference. Indeed, with one-step learning with $n={\cal O}(d^{\ell})$ is only possible if the directions obtained from the gradient with $n={\cal O}(d^{\ell-1})$ are removed, for instance by learning the second layer or pre-processing the data. In contrast, each new step can add a new direction without the need to adapt the second layer weights. 
% %

% The code to reproduce our figures is available on   \href{https://github.com/lucpoisson/GiantStep}{GitHub}, and we refer to App.~\ref{sec:appendix:numerics} for details on the numerical implementations.

% \paragraph{Related Works ---}
% The analysis of high-dimensional asymptotics of kernel regression has provided valuable insights into the advantages and limitations of kernel methods \citep{Dietrich1999, Opper2001, Ghorbani2019, Ghorbani2020, Donhauser2021, Mei2023, Spigler2020, bordelon20a, Canatar2021, simon2022eigenlearning, Cui2021, Cui2022, xiao2022precise}. In particular, a similar stairway picture as in Fig.~\ref{fig:stairway} emerged from these works \cite{xiao2022precise}. The key difference, however, is that at each regime $n={\cal O}(d^{\ell})$, kernels can only learn the $\ell$-th Hermite polynomial of the target. This should be contrasted with our feature learning regime where, once a direction is learned, all its Hermite coefficients are learned. Feature learning corrections to kernel methods have been investigated in \cite{lewkowycz2021the, Naveh2021, Seroussi2023, atanasov2022neural, Bietti2022, bordelon2023dynamics, petrini2022learning}. On a complementary line of work, exact asymptotic results for the the random features models have been derived in the literature \citep{mei_generalization_2022, gerace_generalisation_2020, Dhifallah2020, loureiro_learning_2021, loureiro22a, schroder2023deterministic, bosch2023precise}. A large part of these results are enabled by the Gaussian equivalence property \citep{goldt_gaussian_2021, hu2022universality, Montanari2022, dandi2023universality}.

% In the context of neural network training dynamics, \cite{BenArous2021} established that the sample complexity of learning single-index targets with one-pass SGD is entirely determined by the first non-zero Hermite coefficient, which define an \emph{information exponent}. 

% Closer to us are \citep{ba2022high, damian2022neural}. \cite{ba2022high} showed a sufficiently large single gradient step allows to beat a kernel method. However, their results are limited to single-index target and to a single (giant) gradient step. Here, we build on their results and consider multi-index targets and multiple steps. \cite{damian2022neural} proved that a batch size of $n=d^2$ is \emph{sufficient} for learning multiple directions of a multi-index target. However, they did not establish whether this batch size is \emph{necessary}, and were again limited to a single step. Our results reveal that a batch size of $n=\cO(d^2)$ is indeed necessary for learning multiple directions in a single step, and we characterize which class of multi-index targets can be instead learned with $n=O(d)$ with multiple steps.

% In a related but different vein, \cite{abbe2022merged}, building upon the earlier work of \cite{abbe2021staircase} show how a ``staircase" property of target functions characterizes the sample complexity arises for infinite width two-layer networks trained by one-pass SGD, a.k.a. the mean-field regime \cite{mei2018mean,chizat2018global,rotskoff2018trainability,sirignano2020mean}). Their focus, however, was on the peculiar case of {\it sparse boolean functions} depending solely on linear coefficients, without considering direction-specific specialization.  More recently, \cite{abbe2023sgd} provided partial results for the case of isotropic Gaussian data, always in the regime of one-pass SGD. Here we consider the more generic case of multi-index target functions with Gaussian data with large-batch SGD, and show that a ``directional staircase" behavior arises when iterating a few giant gradient steps, while a related, but definitely different, picture arises with single steps depending on the batch size.

% Finally, our results illustrate that during the early stage of training, neural networks first learn a single direction and require the learning of the linear part of the target function before specializing. This corroborates the findings of \cite{kalimeris2019sgd}, who showed that the neural network first fits the best linear classifier and subsequently learns functions of increasing complexity.


==> sections/investigation.tex <==





% \begin{figure}[t]
%     \centering
%     \includegraphics[width = 1\textwidth]{figs/multiple_steps.pdf}
% %    \vspace{-10em}
%     \caption{{\bf The gradient after multiple steps:}   \lp{Will be put after multiple GD statement. If the proof problem for multiple GD steps cannot be settled, this will be numerics in support of a conjecture for $T<c \log{d}$.} Illustration of the lack of specialization after finite number of GD steps in the proportional regime $n = \mathcal{O}(d)$. We study the cosine similarity with respect to the teacher vectors $(\vec{\theta}_1,\vec{\theta}_2)$ for the gradient of $2$ different neurons (identified respectively by a square and triangle). We fix the relevant dimension $(n,d,p) = (2^{13},2^{13},2^{6})$,  and we perform $15$ GD steps with a fixed learning rate $\eta = \sqrt{p}$. We plot the predicted orientation for the neurons in the teacher subspace as a continuous red line, while the bisectrix of the first quadrant is in a dashed black line. We draw the circle of unitary radius in black, if the gradient was perfectly correlated with the teachers, the neurons would lie on the circumference. On the other hand, the green circle is of radius $\sfrac{2}{\sqrt{d}}$, if the gradient was completely uncorrelated with the teacher, the neurons would lie approximately inside the latter circle. The purple boxes are the end-points for perfectly specialized neurons. We consider different teacher-student settings by fixing the student non-linearity to be $\sigma(z) = \rm{relu}(z)$ and varying the teacher ones for the different sections. Let for simplicity $s(z) = 4z+z^2$, we have: \textbf{Left:} $\sigma_1^*(z) = z, \sigma^*_2(z) = s(z)$. \textbf{Center:} $\sigma_1^*(z) = \sigma^*_2(z) = s(z)$. \textbf{Right:} $\sigma_1^*(z) = s(z), \sigma^*_2(z) = z $.}
%     \label{fig:no_spec}
% \end{figure}


==> sections/theory.tex <==
\subsection{Preliminaries}
%\bl{I think this should go to the appendix}

Before stating our main results, we recall a few definitions and useful facts.
\paragraph{Hermite expansion ---}  Given the Gaussian measure $\gamma_m$ on $\dR^m$, we can build a scalar product on $\ell^2(\dR^m, \gamma_m)$ as
\begin{equation}
    \langle f, g \rangle_\gamma = \int_{\dR^m} f g \ \mathrm{d} \gamma_m = \dE_{\vec{z}\sim \cN(\vec{0}, I_m)}[f(\vec{z})g(\vec{z})].
\end{equation}
It turns out that there is a specific orthonormal basis of interest for this scalar product, that we present in tensor form:
\begin{definition}[Hermite decomposition]\label{def:hermite}
    Let $f: \dR^m \to \dR$ be a function that is square integrable w.r.t the Gaussian measure. There exists a family of tensors $(C_j(f))_{j\in\dN}$ such that $C_j(f)$ is of order $j$ and for all $\vec{x} \in \dR^m$,
    \begin{equation}
        f(\vec{x}) = \sum_{j \in \dN} \langle C_j(f), \cH_j(\vec{x}) \rangle
\label{eq:hermite_expansion}
    \end{equation}
    where $\cH_j(\vec{x})$ is the $j$-th order Hermite tensor \citep{grad_1949_note}.
\end{definition}

\paragraph{Higher-order singular value decomposition ---}

The higher-order singular value decomposition (HOSVD) \citep{de2000multilinear} of a tensor is defined as follows:
\begin{definition}[Higher-order SVD \citep{de2000multilinear}]
    Let $C \in \dR^{m^k}$ be a symmetric tensor of order $k$. A higher-order SVD of $C$ is an orthonormal set $(\vec{u}_1, \dots, \vec{u}_r)$ of $r \leq m$ vectors, as well as a tensor $S \in \dR^{r^k}$ such that
    \begin{equation}
        C = \sum_{j_1, \dots, j_k = 1}^r S_{j_1, \dots, j_k} \vec{u}_{j_1} \otimes \dots \otimes \vec{u}_{j_k},
    \end{equation} 
where $r$ is chosen to be minimal.
\end{definition}
The rank $r$ and the singular values tensor $S$ are unique while like in the case of SVD for matrices, the vectors $(\vec{u}_1, \dots, \vec{u}_r)$ are only unique up to signs, and in the case of identical singular values up to rotations within the corresponding singular value subspace. Furthermore the core tensor $S$ is satisfies all-orthogonality \citep{de2000multilinear}.



% \comment{Reviewer 1 asks for additional clarity on this definition: a) is $m<k$ and not $r<k$?; b) is r minimal in some sense?; c) why also higher-order SVD unique up to rotations. [Yes $r$ is minimal. Add reference and correct that is only true up to permutations and sign not rotations] }
\subsection{Setting and assumptions}
% We consider fully connected neural networks with $p$ hidden neurons: given $W \in \dR^{p\times d}$ and $\vec{a}\in \dR^p$, the network function is defined as
% \begin{equation}\label{eq:def_2lnn}
% \hat f(\vec{z}; W, \vec{a}) = \frac1{\sqrt{p}}\sum_{i = 1}^{p} a_i \sigma(\langle \vec{w}_i, \vec{z} \rangle) = \frac{1}{\sqrt{p}} a^\top \sigma(W \vec{z}),
% \end{equation}
% where $\sigma$ is the non-linear activation function applied elementwise. We study the performance of learning a distribution $\rho$ on pairs $\vec{z}, y$, which corresponds to minimizing the \emph{population loss}
% \begin{equation}
%     \cR(W, \vec{a}) = \dE_{(\vec{z}, y) \sim \rho}\left[ \cL(\hat f(\vec{z}; W, \vec{a}), y) \right],
% \end{equation}
% where $\cL$ is the chosen loss function. In this work, we will focus on the case of the square loss
% \[ \cL(\hat y, y) = \frac12 \left(\hat y - y \right)^2 \]
Before stating our main results, we introduce the setting and main assumptions required. The first concerns the class of target functions we consider.
\begin{assumption}[Data model]
\label{ass:data}
The training inputs $\vec{z}^{\nu}\in\mathbb{R}^{d}$ are independently drawn from the Gaussian distribution $\cN(0, I_d)$. Further, we assume that the target function $y^{\nu}=f^{\star}(\vec{z})$ depends only on a few relevant directions. In other words, there exists a fixed number of orthonormal vectors $(\vec{w}_1, \dots, \vec{w}_r)$ and a fixed function $g^\star: \dR^r \to \dR$ such that  
    \begin{equation}
        y = f^{\star}(\vec{z}) \coloneqq g^\star(\langle\vec{w_1}^\star,\vec{z}\rangle,\dots, \langle\vec{w_r}^\star,\vec{z}\rangle).
    \end{equation}
\end{assumption}
As we will show later, learning with GD can be seen as a hierarchical process, where depending on the batch size different directions of the target are progressively learned. Next, we define the leap index, a fundamental quantity which precisely parametrizes what are the first directions to be learned.
\begin{definition}[Leap index] \label{def:leap}
Since the input data is Gaussian $\vec{z}\sim\mathcal{N}(0,I_{d})$, the target function admits a decomposition in terms of the Hermite decomposition (see Definition \ref{def:hermite}). We define the \emph{leap index} of the target function $f^{\star}$ as the first integer $\ell > 0$ such that  $C_\ell^{\star} = C_\ell(f^\star) \neq 0$:
\begin{align}
   \ell =  \min \{j\in\mathbb{N}: \langle f^{\star},\cH_j\rangle_{\gamma}\neq 0 \}
\end{align}
\end{definition}
% \comment{[Refer to Information exponent \cite{BenArous2021}, this is just its generalization. Refer to IsoLeap of \cite{abbe2022merged} and our results in next section.]}
For single-index models, the above definition reduces to Information Exponent defined in \cite{BenArous2021}. A generalization of the above exponent to sequential learning of directions is defined in \cite{abbe2023sgd} under ``Leap complexity" and ``Isotropic Leap complexity" . We discuss such sequential learning in Section \ref{sec:few-giant-steps}.

Given a batch of training data $(\vec{z}^\nu, y^\nu)_{\nu=1}^{n}\in\mathbb{R}^{d+1}$ drawn from the model \eqref{ass:data} defined above, we now define how the network weights $(W,a)$ are initialized and updated. 
\begin{assumption}[Training procedure]\label{ass:training}
Consider the following random initialization for the weights:
\begin{equation}\label{eq:sample_archit}
    \sqrt{p} \cdot a_i^0 \overset{i.i.d}{\sim} \Unif([-1, 1]) \!\!\quand\!\! \vec{w}_i^0  \overset{i.i.d}{\sim} \Unif(\cS^{d-1}).
\end{equation}
The distribution of the $a_i$ can be replaced by any other continuous distribution with positive variance. Note that for $p=\cO(1)$, we have $\hat f(\vec{z}; W^{0}, \vec{a}^{0})\neq 0$. To further simplify the analysis, we assume $p$ to be even and further impose the following symmetrization at initialization: 
\begin{equation}
    a_i^0 = -a_{p-i+1}^0 \quand \vec{w}_i^0 = \vec{w}_{p-i+1}^0 \quad \text{for all } i \in [p/2],
\end{equation}
which ensures $\hat f(\vec{z}; W^{0}, \vec{a}^{0})=0$. Note that this simplification is common in the related literature, e.g. \cite{chizat_2019_lazy, damian2022neural}, and is mainly necessary when $p$ is small.
% We consider a symmetric initialization such that the network function is identically zero at the start of training. More precisely, assuming $p$ is even we take:
% \begin{equation}
%     a_i^0 = -a_{p-i+1}^0 \quand \vec{w}_i^0 = \vec{w}_{p-i+1}^0 \quad \text{for all } i \in [p/2]. 
% \end{equation}
% Note that this assumption is common in the related literature, e.g. \cite{chizat_2019_lazy, damian2022neural}, and is mainly necessary when $p$ is small, as the initial network function might not concentrate around zero. Moreover, we consider the following random initialization for the weights:
% \begin{equation}
%     \sqrt{p} \cdot a_i^0 \overset{i.i.d}{\sim} \Unif(\{-1, 1\}) \!\!\quand\!\! \vec{w}_i^0  \overset{i.i.d}{\sim} \Unif(\cS^{d-1}).
%     \label{eq:sample_archit}
% \end{equation}
% The distribution of the $a_i$ can be replaced by any other distribution with positive variance, at least when $p$ grows. 
Given the initial conditions, the weights are trained with the following two-step full-batch gradient descent:
\begin{enumerate}[noitemsep,wide=0pt]
    \item \emph{First layer training}: for every gradient step $t\leq T$, a fresh batch of training data $\{(\vec{z}^\nu, y^\nu)\}_{\nu=1}^n$ is drawn from the model in Assumption \ref{ass:data}, and the first layer weights are updated according to:
    \begin{equation}\label{eq:first_layer_gd_again}
        \vec{w}_i^{t+1} = \vec{w}_i^t -  \frac{\eta}{2n} \sum_{\nu = 1}^n \nabla_{\vec{w}_i} \left(y^\nu - \hat f(\vec{z}^\nu; W^t, \vec{a}^{0})\right)^{2},
    \end{equation}
    Hence, the total sample complexity for this step is $Tn$.

    \item \emph{Second layer training}: once the first layer is trained for $T$ steps, the second layer weights $\vec a$ are trained to optimality on an independent batch of data by performing ridge regression with the features learned in the first step: \begin{equation}\label{eq:second_layer_training}\hat{\vec{a}} = \argmin_{\vec{a}\in \dR^p} \frac{1}{2n} \sum_{\nu = 1}^n \left(y^\nu - \hat f(\vec{z}^\nu; W^{T}, \vec{a})\right)^{2} + \lambda \norm{\vec{a}}^2.
    \end{equation}
\end{enumerate}
Such a separation of the training between the first and second layer is a common setup for the theoretical study of training \citep{damian2022neural, abbe2023sgd, berthier2023learning}, and allows for a more tractable study of convergence. 
Note that we assume resampling of data for the training of the second layer for convenience, while we expect the general picture to hold without resampling albeit with a slightly worse sample complexity. See for instance Theorems $1$ and $3$ in \cite{damian2022neural}.

% \comment{[Clarify that we do assume resampling for second layer training. However, cite Damian that discusses what happens if you do not do it.] }
\end{assumption}
We are now ready to state our main technical results.

\subsection{Single gradient step}
\label{sec:1step}
Our starting point is a {\it single} giant gradient step, and the phenomenology described in Fig.~\ref{fig:fig_1}. The main goal is to determine under which conditions the relevant directions $\Pi^{\star}\vec{z}$ of the target function $f^{\star}$ can be learned with the training procedure introduced in Assumption \ref{ass:training}. Hence, a crucial object in our analysis is given by the projection of the network weights in the space spanned by the target relevant directions:  
\begin{equation}
    \vec{\pi}_i^t = \Pi^{\star} \vec{w}_i^t;
\end{equation}
where $\Pi^\star$ is the orthogonal projection on $V^\star$.

%\bl{Link to generalization result}

Our first result is of a negative nature, showing the impossibility of learning in the data-scarce regime:
\begin{theorem}\label{thm:one_step_lower_bound}
    Let $\ell$ be the leap index of $f^{\star}$ \eqref{def:leap}, and assume that $n = \cO(d^{\ell - \delta})$ for some $\delta > 0$. Then, with probability at least $1 - cpe^{-c(\delta)\log(d)^2}$, there exists a universal constant $c$ such that for any $i\in [p]$,
    \begin{equation}
        \frac{\norm{\vec{\pi}_i^1}^2}{\norm{\vec{w}_i^1}^2} \leq c\,\frac{\polylog(d)}{d^{(1 \wedge \delta)/2}}. 
    \end{equation}
\end{theorem}
In other words, for \emph{every} neuron $i$, only a vanishing fraction of the weight $\vec{w}_i^1$ lies in the target subspace $V^{\star}$. In particular, if $\delta > 1$, this large gradient step does not improve over the initial random feature weights.

On the other hand, when $n = \Omega(d^\ell)$, we are able to characterize exactly what is being learned in one gradient step.

\begin{theorem}\label{thm:one_step_learning}
    Assume that the $\ell$-th Hermite coefficient $\mu_\ell$ of $\sigma$ is nonzero, and set the learning rate
    \begin{equation}
        \eta = p d^{\frac{\ell - 1}{2}}.
    \end{equation}
    Then, with probability at least $1 - ce^{-c\log(d)^2}$, there exists a random variable $X$ independent of $d$ with positive expectation such that
    \begin{equation}
        \frac{\norm{\vec{\pi}_i^1}^2}{\norm{\vec{w}_i^1}^2} \geq  X_i,
    \end{equation}
    where $X_1, \dots, X_p$ are i.i.d copies of $X$. Further, let $\vec{u}_1^{\star}, \dots, \vec{u}_{r_\ell}^{\star}$ be the higher-order singular vectors of $C_\ell^{\star}$, and define
    \begin{equation}
        V_\ell^{\star} = \vect(\vec{u}_1^{\star}, \dots, \vec{u}_{r_\ell}^{\star}).
    \end{equation}
    Then, the projections $\vec{\pi}_i^1$ asymptotically belong to $V_\ell^{\star}$, in the sense that there exists a constant $c$ such that
    \begin{equation}
        \norm{(I - \Pi_{V_\ell^{\star}}) \vec{\pi}_i^1} \leq c\, \frac{\polylog(d)}{\sqrt{d}},
    \end{equation}
    and  for $p \geq r_\ell$, they  span the space $V_\ell^\star$. Concretely, for every $\delta>0$ there exists a constant $C_\delta$ such that with probability $1-\delta$:
    \begin{equation}
        \inf_{v \in  V_\ell^\star}\norm{W^1 v} \geq C_\delta.
    \end{equation}
\end{theorem}

    Note that in the case $\ell = 1$ the learned subspace $V^\star_{\ell}$ is one dimensional and is identified by the first Hermite coefficient of the target $C_1(f^\star)$: this corresponds to the ``linear subspace learning'' regime exemplified in Fig.~\ref{fig:fig_1}. Some aspects of the results above were already present in previous works, with key differences: \cite{ba2022high} shows the existence of a rank-one property of the gradient at initialization for $n = \Theta(d)$, and \cite{damian2022neural} implies the positive part of our result for $n = \Theta(d^2)$, provided that $V_2^{\star} = V^{\star}$ (which corresponds to their Assumption 2). Our theorem allows us to obtain the matching lower bounds, demonstrating their tightness, and provides the generic picture for {\it any higher} powers of $d$. In particular, our results prove a clear separation between the class of functions learned within the $\Theta(d)$ batch-size setting of \cite{ba2022high} and the $\Theta(d^2)$ batch-size setting of \cite{damian2022neural} and establish a general hierarchy of functions requiring increasing batch-size to be learned with a single gradient step. We refer to Appendix \ref{sec:appendix:gd_proofs} for the proofs of the theorems and a more detailed technical discussion.
    
  We note that the weak recovery of the subspace $V^\star_{\ell}$ in Theorem \ref{thm:one_step_learning} alone does not suffice towards achieving vanishing generalization error since $V^\star_\ell$ might be a strict subspace of $V^\star$.
    Even in the case when $V_{\ell}^\star=V^\star$, precise generalization bounds depend on the variability of the weights along $V^\star$ and approximation capacity of $\sigma$. 
    However, we believe that for $V_{\ell}^\star=V^\star$, weak recovery guarantees can be translated to perfect recovery and vanishing generalization errors by using $\alpha d^{\ell})$ samples with $\alpha \rightarrow \infty$ and a suitable choice of $\sigma$. For instance, see \cite{damian2022neural} for such an analysis in the case $\ell=2$, at the cost of additional logarithmic factors. We discussion the relationship between weak recovery and generalization errors further in Section \ref{res:generalisation}.
    
    % \comment{Reviewer 1 asks clarification on the implications that the result has on: a) the full recovery of $V^\star_\ell$ and b) the rest of the target function. [Our definition of weak recovery is consistent. However, we agree that strong recovery is not included. (Mention that one could cover strong recovery using techniques similar to Damian.]}

% \fk{Any other advantage that we have? Did we wrote anything to the referee about this?} 



\begin{figure}[t]
    \centering\includegraphics[width = \textwidth]{figs/figBC2.pdf}
    \vspace{-7.em}
    \caption{{\bf Feature learning after a single step.}  Specialization of hidden units in the $n = {\cal O}(d^{k})$ regime $(k = 2, 3)$. The plots show the cosine similarity of the gradient with respect to the target vectors $(\vec{w}^{\star}_1,\vec{w}^{\star}_2)$ for $p = 40$ different neurons, identified by different markers. The bisectrix of the first quadrant is shown as a continuous black line, the circle of unitary radius in black, and the circle of radius $\sfrac{2}{\sqrt{d}}$ in blue. In the upper panel, $(n,d) = (2^{18},2^9)$, and $(n,d) =(2^{21},2^7)$ in the lower one. 
    \\ We use a $2$-index target $f^{\star}(\vec z ) = \sigma^{\star}(\langle\vec{w_1}^{\star},\vec{z}\rangle) + \sigma^{\star}(\langle\vec{w_2}^{\star},\vec{z}\rangle)$, with matching student: $\sigma(z) = \sigma^{\star}(z)$. \textbf{Left:} $\sigma(z) =  \He_1(z)$. \textbf{Center-Left:} $\sigma(z) = \He_2(z)$. \textbf{Center-Right:} $\sigma(z) =  \He_3(z)$. \textbf{Right:} $\sigma(z) = \He_4(z)$. We observe that if the leap index $\ell = 1$, we only learn a single direction, no matter the data quantity, while for $\ell > 1$ we learn every direction as soon as we reach $n = {\cal O}(d^\ell)$. The small spread observed for $\sigma(z) = \He_4(z)$ and $n = {\cal O}(d^3)$ is due to the small value of $d$ used for the experiments. See details in App.~\ref{sec:appendix:numerics}.} 
    \label{fig:d2_d3_regimes}
    \vspace{-1em}
\end{figure}


% \paragraph{Hermite Decomposition of the Gradient---} We show that the gradient can be decomposed into a series of terms where the $k_{th}$ term contains contributions only from the directions having non-zero 
% $k_{th}$ order Hermite coefficient.
% Next, to prove the lower bound on the generalization, we introduce a Gaussian equivalence principle that allows for the presence of "finite-rank" spikes.
% A crucial assumption in the existing gaussian universality results \cite{hu2022universality} is the approximate-orthogonality of the weight matrix.



% As proven in \cite{ba2022high}, when  $\eta=\c{\cal  O}(1)$, the predicted model after a finite number of gradient steps is effectively linear in the inputs. However, with a large scaling of step-size ($\sqrt{p}$), even one step of gradient allows the model to go beyond the linear regime.
% For $\eta=\omega(\sqrt{p})$, the activations of individual neurons become unbounded.

% Therefore, to the study the regime of feature learning, we restrict ourselve to the scaling $\eta=\c{\cal  O}(\sqrt{p})$.

% We show that the improvements over the linear regime are limited to one-direction. The learned predictor 

% Let $f^{\star}:\mathbb{R}^d \rightarrow \mathbb{R}$ be a target function depending on projections along $r$ orthonormal directions $\theta_1,\cdots,\theta_r$ i.e.:
% \begin{equation}
%     f^{\star}(\bx)=g(\theta_1^\top \bx,\cdots,\theta_r^\top \bx).
% \end{equation}

% Then the tensor product of one-dimensional Hermite polynomials form an orthonormal basis for the Hilbert space $L^2(\mathbb{R}^d,\mathcal{N}(\bm{0},\bm{I}))$.

% Let $a_{i_1,\cdots,i_r}$ denote the Hermite coefficient corresponding to the polynomial $\prod_{j=1}^rHe_{(i_j)}(\theta_j^\top \bx)$. For instance, when $r=2$ and $\theta_1, \theta_2$ represent the first two coordinate directions $(1,\cdots,0)$ and $(0,1,\cdots,0)$.
% $a_{1,2}$ represents the coefficient of the polynomial $He^{(1)}(x_1)He^{(2)}(x_2)=x_1(x^2_2-1)$.




% \begin{theorem}\label{thm:rank1}

% For any finite number $K$ gradient steps with step size $\eta=\c{\cal  O}(\sqrt{p})$, and $p=\c{\cal  O}(d)$, there exists a sequence of vectors $\bv_n$ satisfying:
% \begin{enumerate}[noitemsep,leftmargin=1em]
%     \item $G_t \approx \eta \bu^t_n\bv_n^\top + W'_t$ where $G_t$ denotes the $t_{th}$ gradient step, and $W'_t$ has approximately orthonormal rows.
%     \item $\theta_i^\top\bv_n \approx \mu_{1,i}$, where $\mu_{1,i}$ denotes the coefficient of the first Hermite polynomial $He_1(\bx_i)$ on the $i){th}$ coordinate.
%     \item $\mathcal{E}_t(\hat{f}_t(\bx)) \geq \norm{f^{\star}_{\perp_v\geq 1}}^2-o_{\mathbb{P},d}(1)$. This provides a lower-bound on the generalization error achieves after a finite number of steps with ${\cal  O}(d)$ samples. $f^{\star}_{\perp_v\geq 1}$ corresponds to the components of the target function under Hermite decomposition containing non-linear dependence on directions orthogonal to $\bv_n$.
% \end{enumerate}

% \end{theorem}

% The above theorem relies on the separation of the effect of each sample along the spike $\bv_n$ and the orthogonal subspace $\bv_n^{\perp}$. 

\subsection{Learning with many steps}
\label{sec:few-giant-steps}
We now move to the effect of multiple gradient steps, as described in Fig.~\ref{fig:fig_2}. As we shall see, while the effect of multiple steps is limited to a subclass of functions, they can be efficiently learned with few iterations. For simplicity, we restrict ourselves to the case $n = {\cal  O}(d)$, although we expect the findings to hold in the other regimes. We unveil the intertwined dependence between representation learning efficiency and a ``directional staircase'' condition. Informally: once a direction is learned by the first-layer weights, the next gradient step uses it as a ladder to learn the next ones, upon the assumption that they are linearly connected (as we will make precise next). The resulting hierarchical learning picture extends to the large batch case (analyzed in \cite{abbe2022merged} for Boolean inputs) and Gaussian data the observations of \cite{abbe2023sgd} specialized in the single-pass SGD with batch one, using basis-dependent projections. Unlike \cite{abbe2023sgd}, both our definition \ref{def:subspace_conditioning} and the training algorithm are basis-independent.  Lastly, our analysis incorporates the effect of the learned output $\hat f(\vec{z}; W^t, \vec{a})$ on the gradient updates, leading to interaction between neurons. 
Such an interaction was incorporated in the mean-field analysis of \cite{abbe2022merged} for boolean inputs, but supressed in \cite{abbe2023sgd}. 

We formalize the hierarchical learning  by introducing the notion of \emph{subspace conditioning}:
\begin{definition}[Subspace conditioning]\label{def:subspace_conditioning}
    Let $V$ be a vector space, and $U \subseteq V$ a subspace. For any function $f: V\to\dR$, and $\vec{x}\in U$, we define the \emph{conditional} function $f_{U, \vec{x}}: U^\bot \to \dR$ as
    \begin{equation}
        f_{U, \vec{x}}(\vec{x}^\bot) = f(\vec{x} + \vec{x}^\bot)
    \end{equation}
\end{definition}
In short, the function $f_{U, \vec{x}}$ corresponds to $f$ ``conditioned'' on the projection of its argument in $U$. Its first Hermite coefficient will be denoted as
\begin{equation}
    \mu_{U, \vec{x}}(f) = \dE_{\vec{x}^\bot \sim \cN(0, I)}\left[\nabla_{\vec{x^\bot}} f_{U, \vec{x}}\right]
\end{equation}
We are now equipped to state our main result describing sequential learning of directions under multiple gradient steps with batch size $n=\Theta(d)$. We denote by $W^{\star} \in \R^{r \times d}$ the matrix with rows $\vec{w_1}^{\star},\cdots, \vec{w_r}^{\star}$. To avoid degeneracy issues, we restrict ourselves to polynomial activations and target functions.
% \comment{Reviewer 1: Assumption $3$ (polynomial activations) and Assumption $5$ in the appendix (bounded derivatives on $\mathbb{R}$) are incompatible [Fixed in the appendix but need to change the exponent of the Orlicz norm everywhere.]} 
\begin{assumption}\label{ass:activ}
Both the student activation $\sigma: \R \rightarrow \R$ and the teacher function $g^{\star}: \R^r \rightarrow \R$ are fixed polynomials with degrees independent of $d,n$.  
Furthermore, $\operatorname{deg}(\sigma) \geq \operatorname{deg}(g^{\star})$.
\end{assumption}

% \comment{Rev 2: Abbe $2022$ Theorem 7 has stronger results on the negative results concerning generalization error when there is no staircase property. The positive part is implied by Theorem 9 (always Abbe $2022$). Reviewer argues that also this statement is stronger as it is proven that the network will fit the function $f_\star$ for almost all function. [Add comparison to Abbe and give it to them.] }
\begin{theorem}
\label{thm:staircase}
    Assume that $n = {\Theta}(d)$, and $\eta > 0,p \in \N$ are fixed.
    Define a sequence of nested subspaces $U^{\star}_0 \subseteq U^{\star}_1 \subseteq \dots \subseteq U^{\star}_t \subseteq \dots$ as 
\begin{itemize}
    \item $U^{\star}_0 = \{0\}$,
    \item for any $t \geq 0$, $U_{t+1}^{\star} = U_t^{\star} \oplus \vect\left( \{ \mu_{U_t^{\star}, \vec{x}}(f^{\star}): \vec{x} \in U_t^{\star}\} \right)$.
\end{itemize} 
Then, under assumptions \ref{ass:training} and \ref{ass:activ}, after $t$ gradient steps of the form \eqref{eq:first_layer_gd}, $W^t$ satisfies the following with high-probability, for all $i \in [p]$:
\begin{enumerate}
\item Let $\bv \in U_{t}^{\star}$, with $\norm{\bv}=1$ be arbitrary. Let $\bv^m=W^{\star}\bv$ denote the components of $\bv$ along the target basis. Then there exists an almost surely positive random variable $X_{i,t,\bv^m,\ba}$, independent of $d,n$ such that  $\abs{\langle \bw_i,\bv \rangle} \geq X_{i,t,\bv^m,\ba}+ O(\frac{\polylog (d)}{\sqrt{d}})$.

\item For any $\bv \in {U^\bot}_{t}^{\star} \cap V^{\star}$, $\abs{\langle \bw_i,\bv \rangle}=O(\frac{\polylog (d)}{\sqrt{d}})$.
\end{enumerate}
Informally, the above statements imply that almost surely over $\ba$, the first layer learns exactly $U^{\star}_{t}$.
\end{theorem}
% \comment{Rev 1: claims that Abbe et al. are able to recover the ``hidden directions'' while this work overclaims his results. [The phrasing is consistent with what we mean]}
It is easy to check that the above Theorem is consistent with Theorems \ref{thm:one_step_lower_bound}  and \ref{thm:one_step_learning} since $f_{\{0\}, \vec{0}} = f$, and $v^{\star}$ is exactly the first Hermite of $f^{\star}$.
We note that due to the dependence between $X_{i,t,\bv^m,\ba}$ for different $i$ through $\ba$,  Theorem \ref{thm:staircase} doesn't directly imply that $W^{t}$ span $U^\star_t$ for a single instance of $\vec{a}$. We believe that such a spanning result can be obtained via a more careful analysis of the independence of polynomials corresponding to the overlaps $\langle \bw_i,\bv \rangle$arising in the proof of Theorem \ref{thm:staircase}.


\paragraph{Examples ---} As an illustration, we work out the subspaces $U_{t}^{\star}$ for simplified versions of the examples in Figure \ref{fig:multiple_steps}. For simplicity, we will take $\vec{w}_k^{\star} = \vec{e}_k$, the $k$-th vector of the standard basis, so that $\langle \vec{w}_k^{\star}, \vec{z} \rangle = z_k$.
\begin{itemize}[wide=0pt]
    \item $f^{\star}(\vec{z}) = z_1 + z_2 + z_1^2 - z_2^2$: the normalized first Hermite coefficient of $f^{\star}$ is $\vec{v}^{\star} = (\vec{e}_{1} + \vec{e}_{2})/\sqrt{2}$, so $U_1^{\star} = \vect(\vec{e}_{1} + \vec{e}_{2})$. Then, we can rewrite $f^{\star}$ in the new basis $(\vec{v}^{\star}, \vec{v}^\bot)$, to get
    \[f^{\star}(\vec{z}) = \sqrt{2}\langle \vec{v}^{\star}, \vec{z}  \rangle + 2 \langle \vec{v}^{\star}, \vec{z} \rangle \langle \vec{v}^\bot, \vec{z} \rangle. \]
    Hence, if $\vec{x} = \lambda \vec{v}^{\star}$, we have $\mu_{U_{t}^{\star}, \vec{x}}(f^{\star}) = 2\lambda \vec{v}^\bot$, and hence $U_2^{\star} = V^{\star}$.

    \item $f^{\star}(\vec{z}) = z_1 + z_2 + z_1^2 + z_2^2$: just as the above example, $U_1^{\star} = \vect(\vec{e}_{1} + \vec{e}_{2})$, and hence we perform the same change of basis. However, this time,
    \[f^{\star}(\vec{z}) = \sqrt{2}\langle \vec{v}^{\star}, \vec{z}  \rangle + \langle \vec{v}^{\star}, \vec{z} \rangle^2 +  \langle \vec{v}^\bot, \vec{z} \rangle^2. \]
    This implies that for any $\vec{x}\in U_1^{\star}$, $\mu_{U_{t}^{\star}, \vec{x}}(f^{\star}) = \vec{0}$, and the direction of $\vec{v}^\bot$ is never learned.
\end{itemize}

We provide a proof of Theorem \ref{thm:staircase} in Appendix \ref{sec:appendix:gd_proofs}. The notion of subspace conditioning (Definition \ref{def:subspace_conditioning}) arises through an inductive decomposition of the projections of the gradient along the target subspace. Furthemore, our theory leads to a precise prediction of the orientation of the gradient in the target subspace after a finite number of steps. This is illustrated in Figure \ref{fig:multiple_steps}. Note that the non-linearity of the activation function allows different neurons to simultaneously specialize along different directions in contrast to the rank-one increase at each saddle in deep linear networks \cite{jacot2021saddle} under vanishing initialization. We refer to Appendix \ref{sec:appendix:numerics} for additional discussion.


To conclude this section, we provide an overview of our present understanding of the effect of batch-size (sample complexity), number of gradient-steps (iteration complexity), and the number of neurons (overparameterization) on learning different multi-index target functions in table \ref{table}. For simplicity, when discussing the leap index $\ell$, we restrict to functions where all the directions in the target subspace have the same leap i.e when $V^*_\ell= V^*$. We define ``staircase functions" as target functions such that the sequence of subspaces defined through subspace conditioning in Theorem \ref{thm:staircase} eventually span $V^*$.

\begin{table}[ht]
\renewcommand{\arraystretch}{1.0}
\begin{center}
 \begin{adjustwidth}{-0cm}{}
\begin{tabular}{||c|| c | c | c ||}
 \hline
 Complexity  & SGD  & One-step GD & Multi-step GD  \\ 
 of $f^*$  & with $n=1$&with $n=\Theta(d^{\ell})$ &with $n=\Theta(d)$\\ 
 \hline Single-index, $\ell\!=\!1$& \textcolor{blue}{$\tau\!=\!n_{\rm{T}}\!=\!d$} & \textcolor{ForestGreen} {$\tau\!=\!1, n_{\rm{T}}\!=\! n \!=\!\Theta(d)$} & $\tau\!=\!1,n_{\rm{T}}\!=\!\Theta(d)$ \textcolor{magenta}{$(\star)$} \\ 
 \hline Single-index, $\ell\!=\!2$ & \textcolor{blue}{$\tau\!=\!n_{\rm{T}}\!=\!d\log d$} & \textcolor{orange}{$\tau\!=\!1,n_{\rm{T}}\!=\!n\!=\!\Theta(d^2)$\!\!\!} & \textcolor{red}{\!\!\!$\tau\!=\!\Theta(\log d),n_{\rm{T}}\!=\!\Theta(d\log d)$}\!\!\! \\
 \hline
 Single-index, $\ell>2$ & \textcolor{blue}{$\tau=n_{\rm{T}}=d^{\ell-1}$} & \!\!\!$\tau=1,n_{\rm{T}}\!=\!n\!=\!\Theta(d^\ell)$\!\!\! & \textcolor{red}{$\tau\!=\!\Theta(d^{\ell-2}),n_{\rm{T}}\!=\!\Theta(d^{\ell-1})$} \\
 \hline 
 Staircase & \textcolor{blue}{$\tau=n_{\rm{T}}=d$} & $\tau\!=\!1,n_{\rm{T}}\!=\!n\!=\!\Omega(d^2)$ & $\tau\!=\!\Theta(1),n_{\rm{T}}\!=\!\Theta(d)$ \textcolor{magenta}{$(\star)$} \\
 \hline 
\end{tabular}
\end{adjustwidth}
\caption{\label{table} Number of iterations $\tau$ and sample complexity $n_{\rm{T}}$ needed to learn the features/directions of the function $f^*$ with SGD one-sample at a time, using a single step-gradient descent, or using one-pass GD with large $n=O(d)$ batches. Results in \textcolor{blue}{(blue)} are from \cite{BenArous2021,abbe2023sgd}. 
% \review{while entries in \textcolor{magenta}{(magenta)} refers to \cite{abbe2022merged} in the Boolean setting}. 
The upper bounds on the sample complexity are known to hold from \textcolor{ForestGreen}{(green)} \cite{ba2022high} and \textcolor{orange}{(orange)} \cite{damian2022neural}, while the corresponding lower bound, as well as the results in black, are proven in the present paper. \textcolor{red}{(red)} are educated guesses, which are out of the scope of the paper since we only focus on a finite number of iterations $\tau$. For staircase functions, one-step GD may require more than $\Theta(d^2)$ samples depending on the maximum leap across directions in the target subspace. 
The marker \textcolor{magenta}{$(\star)$} refers to similar results in \cite{abbe2022merged} for the case of Boolean inputs and extended in the present work for the Gaussian setting.}

\end{center}
\end{table}



\subsection{From feature learning to generalization bounds} 
\label{res:generalisation}


\begin{figure}[t]
    \centering    
\includegraphics[width = 1\textwidth]{figs/multiple_steps.pdf}
   \vspace{-5em}
    \caption{{\bf Feature learning with multiple gradient steps.} 
    \textbf{Top:} Generalization error as a function of $n$ ($d=512,p=256$) after iterating the training procedure for six steps. \textbf{Bottom:} Cosine similarity of the projected gradient matrix $G^p$ inside the target subspace for all the $p$ neurons at a fixed ratio $\sfrac{n}{d} = 4$, plotted at different stages of the training. The blue and purple lines are the theoretical predictions for the orientation of the gradient in the second step. \\
        We fix a \rm{relu} student and consider two different 2-index target functions $f^{\star}(\vec z) = \sigma^{\star}_1(\langle\vec{w_1}^{\star},\vec{z}\rangle) + \sigma^{\star}_2(\langle\vec{w_2}^{\star},\vec{z}\rangle)$. {\bf Left:} $\sigma^{\star}_1(z) = \sigma^{\star}_2(z) = \He_1(z) + \sfrac{\He_2(z)}{2} + \sfrac{\He_4(z)}{4!}$ \quad{\bf Right:} $\sigma^{\star}_1(z) = z-z^2$ and $\sigma^{\star}_2(z) = z+ z^2$. In accordance with Theorem \ref{thm:staircase}, the difference between the two cases is clear already after the first GD step: while on the left the gradient is stuck around the predicted rank-one spike after the first step (black line), on the right the gradient changes orientation in the second step, allowing to learn multiple features. See details in App.~\ref{sec:appendix:numerics}.}
    \label{fig:multiple_steps}
    \vspace{-1em}
\end{figure}


We now investigate the consequence of Theorem \ref{thm:one_step_learning} in the actual performance of the neural network. At a high-level, one expects that learning a subspace $U$ by the first-layer effectively reduces the input-dimensionality to that of $U$, allowing the network to learn a function dependent on $U$ using a significantly fewer number of examples and neurons. However, for learning functions dependent on directions not yet learned by $W$, we expect a requirement of a large number of neurons as well as samples, analogous to the setting of random features. In the following, we make this intuition precise by proving that the generalization error of training the second layer on the top of the learned features is lower bounded precisely by the directions which were not learned by the first-layer. Our results and conjectures incorporate the dependence on both the number of samples and the number of hidden neurons.





% This is a fairly complex question: indeed,  \fk{This should be said later, in the finite p regime we cannot learn anything.}
 

\paragraph{Finite $p$ regime ---} This is the simplest case: in this setting, there is simply no way to fit anything beyond the learned directions, even with an infinite amount of data. This is formalized by the following proposition:
\begin{proposition}\label{prop:fixed_width_lower_bound}
    Assume that $p$ is bounded as $n, d \to \infty$, and that the first layer $W$ only learns a subspace $U \subseteq V^{\star}$, i.e for any $v \in V^{\star}, v \perp U$, $\abs{\langle \vec{w}_i, \vec{v} \rangle} = o(1)$.
    For any choice of second layer $\vec{a}$ such that $\norm{\vec{a}}_\infty \leq {\cal  O}(1)$, we have
    \begin{equation}
    \dE\left[\left(f^{\star}(\vec{z}) - \hat f(\vec{z}; W, \vec{a})\right)^2\right] \geq \dE\left[\Var\left( f^{\star}(\vec{z})   \mid P_U \vec{z}\right)\right] - o(1)
    \end{equation}
    where $P_U$ is the orthogonal projection on $U$.
\end{proposition}
% \comment{Reviewer 1: What does it mean to ``learn'' a subspace $U$? Look at Appendix $C.1$ it means $|| P_{U^\perp} w_i|| < \varepsilon_d$ but that would be a stronger notion of recovery than the ``weak recovery'' one guaranteed by the above theorems. [It does not assume strong recovery it only assumes absence of weak recovery in other directions in the teacher subspace. We will revise the notation for $U^\perp$ as it is not the true complement but only restricted to the teacher subspace.]}

We refer to Appendix \ref{sec:appendix:cget_proofs} for the proof of the proposition.
In particular, Proposition \ref{prop:fixed_width_lower_bound} implies that with bounded $p$, the model cannot achieve vanishing generalization error unless $U=V^\star$. For Boolean data, such a lower-bound in the absence of recovery of the full-subspace was proven in Theorem 9 of  \cite{abbe2022merged}. Proposition \ref{prop:fixed_width_lower_bound}, however provides a fine-grained lower bound for any $U \subseteq V$. 

Intuitively, the right-hand side of the above inequality corresponds to the predictor $\hat f(\vec{z}) = \dE\left[ f^{\star}(\vec{z}) \mid P_U \vec{z} \right]$, which is the best predictor that depends only on $P_U \vec{z}$. Conversely, we expect that with enough neurons, it is possible to approximate this predictor:
\begin{conjecture}
\label{conj:approxim_conj}

Suppose that $n=\alpha d^\ell$ in Theorem \ref{thm:one_step_learning} or $n=\alpha d$ in Theorem \ref{thm:staircase}. For any  $\delta > 0$, there exists a $p_0 \in\dN$ and $\alpha_0 \in \R^+$ such that if $p \geq p_0$, $\alpha \geq \alpha_0$, there exists a choice of second layer $\vec{a}$ satisfying $\norm{\vec{a}}_\infty \leq {\cal O}(1)$, such that as $n, p \to \infty$
    \begin{equation}
        \dE\left[\left(f^{\star}(\vec{z}) - \hat f(\vec{z}; W, \vec{a})\right)^2\right] \leq \dE\left[\Var\left( f^{\star}(\vec{z})   \mid P_U \vec{z}\right)\right] + \delta + o(1)
    \end{equation}
\end{conjecture}

%\fk{We need to say why we are not proving it, and why it hard, and how Damian et al are VERY SPECIFIC!! Again, use what we say to the referee}
% \comment{Mention that Abbe $2022$ has already proven this phenomenon in the Boolean setting (Theorem 9) and that numerical investigation also in the Gaussian cases was provided. [It is finite $p$ so we should give it to Abbe.]}
Proving the above conjecture for generic target and activation functions requires proving a sufficient spread of $W$ along the learned subspace $U$ together with an approximation result for finite-dimensional neural networks having activation function $\sigma$. 
Such a conjecture is proven in \cite{damian2022neural} for the specific case of $U = V^{\star}$ (in which case the first term in the RHS is zero) and $\sigma = \operatorname{relu}$, with an additional bias term, and in Theorem $9$ of \cite{abbe2022merged} for Boolean inputs with activation $\sigma(x)=(1+x)^L$ for a particular choice of $L$
For generic $\sigma$ with Gaussian inputs, such approximation results are scarcer. In particular, since the projection of the weights $W$ along $U$ cannot be chosen arbitrarily, one cannot directly invoke classical approximation results such as the ones based on Barron spaces. However, the components of $W$ along $U$ are still randomly distributed across neurons. Therefore, one possible approach could be to use results on the generalization of random feature models on finite-dimensional inputs such as \cite{rudi2017generalization}. We leave such an analysis for future work.


\begin{wrapfigure}{r}{0.46\textwidth}
  \vspace{-0.6cm}
% \begin{figure}[t!]
%        \centering
%        \begin{minipage}[c]{0.46\textwidth}
            \includegraphics[width=0.45\textwidth]{figs/example.pdf}
%        \end{minipage}
%        \hfill
%        \begin{minipage}[c]{0.52\textwidth}
%            \vspace{-0.2cm}
            \caption{{\bf Learning with training of the second layer.} Simulation illustrating the different regimes in Fig.~\ref{fig:fig_1}, using $d\!=\!512, p\!=\!1024$, a symmetric two-index target function $f^{\star}(\vec z) = \sigma^{\star}(\langle\vec{w_1}^{\star},\vec{z}\rangle) + \sigma^{\star}(\langle\vec{w_2}^{\star},\vec{z}\rangle)$ with activation $\sigma^{\star}(z)=\He_1(x)+\He_2(x)/2!+\He_4(x)/4!$, and a \rm{relu} student. (a) The first algorithm (green) applies a giant step and then learns the second layer. When $n\!\gg\!d$, its performance goes beyond the linear predictor that would be obtained with a kernel method and reach the ``linear subspace learning'' regime in Fig.~\ref{fig:fig_1}. (b)  To go beyond this regime, the second algorithm (blue) preprocesses the data to remove a plug-in estimate of the first Hermite coefficient. It reaches a lower plateau as $n\!\approx\!d^2$, now beating the quadratic kernel. We contrast this behavior with the one of the random feature model (red). Details can be found in App.~\ref{sec:appendix:numerics}.}
        \label{fig:example}
%        \end{minipage}
%        \hfill
       \vspace{-2em}
%    \end{figure}
\end{wrapfigure}

\paragraph{Beyond the fixed width regime ---} 
%
When the number of neurons is allowed to diverge, it is no longer impossible to learn funtions along the directions that are not present in $U$. Indeed, \cite{Mei2023} shows that even in the absence of feature learning (i.e. when the first layer is random), it is possible to learn a polynomial approximation of $f^{\star}$ of degree $k$ as long as $n, p = \Omega(d^{k + \delta})$ for some $\delta > 0$. The exact performance of the network may heavily depend on the training process for the second layer. Intuitively, we expect the following behavior: 
\begin{enumerate}[noitemsep,leftmargin=1em,wide=0pt]
    \item On the directions present in $W$, with enough variety in the neurons, the model behaves similarly as a random feature one in this {\it finite}-dimensional space, and are thus able to learn ``everything''.
    \item On the orthogonal directions, however, the models still behave as a random feature model in high dimension, and thus the polynomial limitations of \cite{Mei2023} still apply.
\end{enumerate}
To formalize this conjecture, we introduce the following definition:
\begin{definition}
    Let $V$ be a vector space, and $U \subseteq V$ a subspace. For any $k \geq 0$, we define the space $\cP_{U, k}$ of functions $f: V \to \dR$ such that for any $\vec{x}\in U$, the function $f_{U, \vec{x}}$ introduced in Definition \ref{def:subspace_conditioning} is a polynomial of degree at most $k$.
\end{definition}

Simply put, the space $\cP_{U, k}$ consists of polynomials in $\vec{x}^\bot$ of degree at most $k$, whose coefficients can be functions of $\vec{x}$. We will denote by $P_{U, \leq k}$ and $P_{U, >k}$ the projections on $\cP_{U, k}$ and $\cP_{U, k}^\bot$ in $\ell^2(\dR, \gamma)$, respectively, where $\gamma$ is the Gaussian measure. 
This allows us to write the above intuition in the following precise conjecture:
\begin{conjecture}\label{conj:kernel+feature}
    Assume that $p = {\cal O}(d^{\kappa_1})$ and $n = {\cal O}(d^{\kappa_2})$, and that the first layer $W$ only learns a subspace $U^{\star} \subseteq V^{\star}$.    Then, if $\hat{\vec{a}}$ is obtained as in Eq. \eqref{eq:second_layer_training} for any value of $\lambda$,
    \begin{equation}
        \dE\left[\left(f^{\star}(\vec{z}) - \hat f(\vec{z}; W, \hat{\vec{a}})\right)^2\right] \geq \norm{P_{U^{\star}, >\kappa} f^{\star}}^2_\gamma - o(1),
    \end{equation}
    where $\kappa = \min(\kappa_1, \kappa_2)$ and $\norm{}_\gamma$ is the norm in $\ell^2(\dR, \gamma)$.
\end{conjecture}
While a general proof for this conjecture would require significant additional work, we can prove some particular cases. First, it is easy to check that Proposition \ref{prop:fixed_width_lower_bound} corresponds to the $\kappa = \kappa_1 = 0$ case of the above conjecture. Second, in the next section, we prove the fairly delicate $\kappa_1 = \kappa_2$ case.

\paragraph{The linear case ---} We provide a proof of the $\kappa_1 = \kappa_2 = 1$ case of the above conjecture, also known as the \emph{proportional regime}. In this setting, \citep{mei_generalization_2022, gerace_generalisation_2020, goldt_gaussian_2021, hu2022universality} have shown that for the random features $W^{0}$ case, the generalization error of the minimizer for the second layer \eqref{eq:second_layer_training} is equivalent to the generalization error of an equivalent linear model; this result was extended in \cite{ba2022high} to a trained first layer $W^{1}$ for small, ``lazy'' stepsizes $\eta = {\cal O}(1)$.
%
\cite{ba2022high} has also shown that when $\eta = \Theta(p)$, the equivalent linear description breaks down, due to the appearance of a spike term proportional to $\eta$ in the trained weight matrix $W^{1}$; here, we show that this spike only allows the learning of non-linear functions parallel to the spike. Notice that the optimization problem \eqref{eq:second_layer_training} is equivalent to
\begin{equation}\label{eq:ck_kernel}
    \min_{\vec{a} \in \dR^p} \frac1n \sum_{\nu = 1}^n \left( \langle \vec{a}, \phi_{\text{CK}}(\vec{z}^\nu)\rangle - f^{\star}(\vec{z}^\nu) \right)^2 + \lambda \norm{\vec{a}}^2
\end{equation}
where $\phi_{\text{CK}}(\vec{z}) = \sigma(W\vec{z})$ is the feature map corresponding to the \emph{conjugate kernel} of the neural network. For a given direction $\vec{v}$, we define the \emph{conditional linear} equivalent map $\phi_{\text{CL}}(\vec{z}; \vec{v})$ as follows: given the decomposition $\vec{z} = z_{\vec{v}} \vec{v} + \vec{z}^\bot$,
\begin{equation}
    \phi_{\text{CL}}(\vec{z}; \vec{v}) = \mu\left(z_{\vec{v}}\right) + \Psi(z_{\vec{v}}) z^\bot +  \Phi(z_{\vec{v}})\vec{\xi}
\end{equation}
where $\vec{\xi} \sim \cN(0, I_p)$, and $\mu\in\dR^p, \Psi\in \dR^{p\times d}, \Phi \in \dR^{p \times p}$ are chosen to match the first two conditional moments of $\phi_{\text{CK}}$:
\begin{align*}
    \mu(z_{\vec{v}}) &= \dE\left[ \phi_{\text{CK}}(\vec{z}) \mid z_{\vec{v}} \right], \quad\Psi(z_{\vec{v}}) = \dE\left[ \phi_{\text{CK}}(\vec{z})(z^\bot)^\top \mid z_{\vec{v}} \right],\\ 
    \Phi(z_{\vec{v}}) &= \Cov\left[ \phi_{\text{CK}}(\vec{z}) \mid z_{\vec{v}} \right] - \Psi(z_{\vec{v}})\Psi(z_{\vec{v}})^\top
\end{align*}

Then, the following theorem holds:

\begin{theorem}\label{thm:cget}(informal)
     Assume that $n, p = \Theta(d)$, and that $V_1^\star$ defined in Theorem \ref{thm:one_step_learning} is non-zero. Let $v^\star=C_1(f^\star)$, so that $V_1^\star = \vect(v^\star)$.Then, after one gradient step, there exists a vector $\vec{v} \in \dR^d$ such that:
    \begin{itemize}[noitemsep,wide=0pt]
        \item the projection of $\vec{v}$ on $V^{\star}$ is proportional to $\vec{v}^{\star}$,
        \item the solutions $\hat{\vec{a}}$, $\tilde{\vec{a}}$ to the optimization problem in \eqref{eq:ck_kernel} with the feature maps $\phi_{\text{CK}}(\vec{z})$ and $\phi_{\text{CL}}(\vec{z}; \vec{v})$ yield the same generalization error.
    \end{itemize}
\end{theorem}
The full statement of Theorem \ref{thm:cget} with the relevant hypotheses is discussed App.~\ref{sec:appendix:cget_proofs}. In particular, as we show in App.~\ref{sec:appendix:cget_proofs}, Theorem \ref{thm:cget} provides a proof of the case $\kappa_1 = \kappa_2 = 1$ of Conjecture \ref{conj:kernel+feature}:
\begin{corollary}\label{corr:lower_bound}
Conjecture \ref{conj:kernel+feature} holds for $\kappa_1 = \kappa_2 = 1$.
\end{corollary}
Informally, as for the random features model, features in the subspace orthogonal to $\vec{v}$ map to a linear model, and therefore only the linear part of $f^{\star}$ can be learned in this subspace. This precisely corresponds to the statement in Conjecture \ref{conj:kernel+feature}. This is illustrated in particular in Fig.\ref{fig:features} where the generalization after one step of gradient descent is improved  drastically over initialization for $f^\star(\vec z)=z_1+z_1 z_2$, while it is not for $f^\star(\vec z)=z_1+z_2 z_3$. 
% Fig.\ref{fig:postive_cget_appendix} illustrates this phenomenon for more complex functions $f^\star(\vec z)=z_1+z_1z_2+g_{3}(z_1)z_3$ vs $f^\star(\vec z)=z_1+z_2z_3+g_{3}(z_2)z_3$, where $g_{\ell}$ is an auxiliary function with leap index $\ell$ (See App.~\ref{sec:appendix:numerics}). 
We refer to App.~\ref{sec:appendix:numerics} for additional discussion on the numerical validation of these claims. 

\paragraph{General overview ---} We conclude this section by offering a summary on the generalization properties of two-layer networks. In table \ref{table2} we focus on the effect of overparameterization, i.e. number of neurons in the hidden layer. 
% \begin{table}[h]
% \renewcommand{\arraystretch}{1.20}
% % \begin{center}
% \begin{tabular}{|c||c | c | c ||}
%  \hline
%  $f^*$ & Random Features & One-step GD & Multi-step GD \\
%  \hline  $z_1+z_1z_2$ &$ \min (p,n) \!=\! \tilde{\Theta}(d^2)$ & $p\!=\!\Theta(d),n\!=\!\Theta(d)$ &$\tau\!=\!2,p\!=\!\Omega(1),n\!=\!\Theta()$\\ 
% \hline  $z_1+z_2z_3$ &$ \min (p,n) \!=\! \tilde{\Theta}(...)$ & $p\!=\!\Theta(...),n\!=\!\Theta(d)$ &$\tau\!=\!3,p\!=\!\Theta(...),n\!=\!\Theta(...)$\\ 
%  \hline
%   $z_1+z_1z_2+g_{3}(z_2)z_3$ &$ \min (p,n) \!=\! \tilde{\Theta}(d^3)$ & $p\!=\!\Theta(d),n\!=\!\Theta(d)$ & $\tau\!=\!2,p\!=\!\Theta(1),n\!=\!\Theta(d)$\\ 
%  \hline  $z_1+z_2z_3+g_{3}(z_2)z_3$ &$ \min (p,n) \!=\! \tilde{\Theta}(...)$ & $p\!=\!\Theta(...),n\!=\!\Theta(d)$ &$\tau\!=\!3,p\!=\!\Theta(...),n\!=\!\Theta(...)$\\ 
%  \hline 
% \end{tabular}
% \caption{\label{table2}: \textcolor{blue}{LP: Running the third row, to include a new positive example looking at 2GD steps.} Sample complexity $n_{\rm{T}}$ required to fit a target function upto a desired accuracy. Random Features correspond to $\tau=0$ i.e the network at initialization.}
% % \end{center}
% \end{table}

%%% New attempt %%%% 
\begin{table}[h]
\renewcommand{\arraystretch}{0}
 \begin{adjustwidth}{0cm}{}
\begin{tabular}{||c||c || c | c ||}
 \hline
 $f^*(\cdot)$ & Random  & GD & GD   \\
  & Features & $p\!=\!\mathcal{O}(1), n\!=\!\mathcal{O}(d)$& $p\!=\!\mathcal{O}(d), n\!=\!\mathcal{O}(d)$ \\
 \hline 
  \hline  $z_1\!+\!z_1z_2$ &$ \min (p,n) \!=\! \tilde{\Theta}(d^2)$ & $\tau = 2$ &$\tau = 1$\\ 
\hline  $z_1\!+\!z_2z_3$ &$ \min (p,n) \!=\! \tilde{\Theta}(d^2)$ &\!No learn. in $\tau\!=\!\Theta(1)$\!&\!No learn. in $\tau\!=\!\Theta(1)$\!\\
 \hline $z_1\!+\!z_1z_2\!+\!\He_{3}(z_1)z_3$ &$ \min(p,n) \!=\! \tilde{\Theta}(d^4)$ & $\tau = 2$ & $\tau = 1$\\ 
\hline  $z_1\!+\!z_1z_2\!+\!\He_{3}(z_2)z_3$ &$ \min (p,n) \!=\! \tilde{\Theta}(d^4)$ & $\tau = 3$ &$\tau = 2$ \\
\hline  $z_1\!+\!z_2z_3\!+\!\He_{3}(z_2)z_3$ &$ \min (p,n) \!=\! \tilde{\Theta}(d^4)$ &\!No learn. in $\tau\!=\!\Theta(1)$\!&\!No learn. in $\tau\!=\!\Theta(1)$\!\\
 \hline 
\end{tabular}
\end{adjustwidth}
\caption{\label{table2}\textbf{Overparametrization helps learning multi-index targets.} Table summarizing the number of iterations needed to learn different multi-index targets $f^\star(\cdot)$  with underparametrized $\left(p = \mathcal{O}(1)\right)$ and overparametrized $\left(p=\mathcal{O}(d)\right)$ two-layer networks trained in the proportional batch-size regime $n=\mathcal{O}(d)$. We contrast this behaviour with the sample complexity of Random Features trained with $n$ samples ($n_{\rm{T}}=n$), corresponding to $\tau=0$, i.e, the network at initialization. The time complexity can be significantly reduced by considering overparametrized networks, in accordance with Theorem~\ref{thm:cget}.}
\end{table}
Here, the function $f^\star(\vec{z})=z_1+z_1z_2$ can either be learned in two steps through the staircase property or in a single step by increasing the number of hidden neurons. This is an example of a multi-index target function that can be learned with a single step of $\mathcal{O}(d)$ batch-size through overparameterization, exemplified in the left panel of Fig.~\ref{fig:features}. On the other hand, $f^\star(\vec z) = z_1 + z_2z_3$ is not linear conditioned on $z_1$ (learned at the first step), and this leads to a generalization pattern similar to Random Features in the overparametrized regime, see right panel of Fig.~\ref{fig:features}. We refer to App.~\ref{sec:appendix:numerics} for the analysis of the last two example of Table~\ref{table2} (see Fig.~\ref{fig:postive_cget_appendix}). 
\\Conjecture.~\ref{conj:kernel+feature} extends the claims of Thm~\ref{thm:cget} to the polynomial scaling regime of $p = \mathcal{O}(d^{\kappa_1})$ and $d = \mathcal{O}(d^{\kappa_2})$. We exemplify the effect of overparametrization in this setting by considering the following target function:
\begin{equation}
f^\star(\vec{z})=z_1+\He_3(z_1)z_2+\He_2(z_1)\He_2(z_3).
\end{equation}
Here, we can illustrate the intertwined dependence between batch-size, number of hidden neurons, and time iteration in determining learning efficiency. Indeed, changing any of these quantities can affect the components of the target function that are fitted by the network. Consider the following concrete scenarios, where $\hat{f}(\vec{z})$ denotes the predicted output function, after training the second layer:
\begin{enumerate}
    \item One-step GD with $n =\Theta(d), p = \mathcal{O}(1)$: $\hat{f}(\vec{z})=z_1$.
    \item One-step GD with $n =\Theta(d), p = \mathcal{O}(d)$: $\hat{f}(\vec{z})=z_1+\He_3(z_1)z_2$.
    \item One-step GD with $n = \Theta(d^2)$, $p = \Theta(d^2)$: $\hat{f}(\vec{z})=z_1+\He_3(z_1)z_2+\He_2(z_1)\He_2(z_3)$. 
    % Here one gradient step is performed with batch-size $\Theta(d)$ and subsequently the second layer is trained using $\Theta(d^2)$ samples.
\end{enumerate}
% For the sake of clarity we used Hermite polynomials in the discussion, but we did not consider them in the experiments to produce Fig.~\ref{sec:appendix:numerics}. This choice improves numerical stability of simulations and we refer to App.~\ref{sec:appendix:numerics} for additional details on the numerics.
%\subsection{Discussion}

%\paragraph{Sample and time complexity of large batch learning} The complexity of learning a low-dimensional teacher function (or even a single-index model) is a topic that recently saw a surge of interest. For a single-index function with leap index $\ell$, it is known that one-pass SGD has a sample complexity of $\cO(d^{\ell - 1})$ \citep{BenArous2021}, and it has been recently shown \citep{damian_2023_smoothing} that a smoothed version of SGD achieves a sample complexity of $\cO(d^{\ell/2})$. This matches a lower bound from the correlation statistical query family, which encompasses all SGD-like methods. In our setting, we showed in Theorems \ref{thm:one_step_lower_bound} and \ref{thm:one_step_learning} that the sample complexity for large batch learning is $\cO(d^\ell)$, which is worse than both the above methods.

% However, the time complexity of each algorithm paints a different picture. Both SGD algorithms are sequential, and require $\cO(d)$ operations per step, which leads to a total time complexity of $\cO(d^{\ell/2 + 1})$ at minimum. On the other hand, the computation of the update in eq. \eqref{alg:gd_training} is simply an average of independent terms, which is very easy to parallelize. Including the time to compute the average of each term e.g. using a Gossip algorithm \cite{boyd_2006_randomized}, this sums up to a time complexity of $\cO(d + \log(n))$. Such an algorithm is also very amenable to decentralized learning schemes, where each agent only has access to a fraction of the overall data.

\section*{Conclusion}
% \comment{[Cite the ICML work Arnaboldi et al. that originated from the conjecture in Table 2]. [Add discussion on strong recovery and that one could expand using techniques coming from Damian]}
In this work, we investigated the dynamics of two-layer neural networks as they learn a multi-index model using a single-pass, large-batch, gradient descent algorithm. We shed light on the intricate interactions between the task's structure, notably the complexity of the target function, the hyperparameters of SGD, such as the batch size and learning rate, and the network architecture, such as how the hidden layer width impact the approximation capacity of the network at fixed data budget. We highlight three key findings: a) The pronounced influence of a single gradient step on feature learning, underlining the nexus between batch size and the target's information exponent; b) The amplification of the network's approximation capacity over successive gradient steps and the learning of increasingly complex functions over time; c) The improvement in generalization when contrasted with the random feature/kernel regime. In conclusion, we presented a thorough mathematical framework detailing many nuances of data representation learning in two-layer neural networks during their early training phase. Finally, we note that while certain aspects of those results are left as conjectures, we believe that they capture both the dynamics of multiple gradient steps, as well as the structure of the remaining directions. Proving those conjectures requires fairly delicate concentration and random matrix arguments, which may be of independent mathematical interest.



\section*{Acknowledgements}
We thank Denny Wu, Theodor Misiakiewicz, Loucas Pillaud-Vivien, Joan Bruna \& Lenka Zdeborov\'a for insightful discussions. We also acknowledge funding from the Swiss National Science Foundation grant SNFS OperaGOST, $200021\_200390$ and the \textit{Choose France - CNRS AI Rising Talents} program.
